A semi-implicit dynamical low-rank discontinuous Galerkin method for space homogeneous kinetic equations. Part I: emission and absorption

Dynamical low-rank approximation (DLRA) is an emerging tool for reducing computational costs and provides memory savings when solving high-dimensional problems. In this work, we propose and analyze a semi-implicit dynamical low-rank discontinuous Galerkin (DLR-DG) method for the space homogeneous kinetic equation with a relaxation operator, modeling the emission and absorption of particles by a background medium. Both DLRA and the DG scheme can be formulated as Galerkin equations. To ensure their consistency, a weighted DLRA is introduced so that the resulting DLR-DG solution is a solution to the fully discrete DG scheme in a subspace of the classical DG solution space. Similar to the classical DG method, we show that the proposed DLR-DG method is well-posed. We also identify conditions such that the DLR-DG solution converges to the equilibrium. Numerical results are presented to demonstrate the theoretical findings.

==> LiteratureReview.tex <==
\section{Literature Review}

==> archive/Background12082022.tex <==
\section{Background}

\subsection{Model Equations}

The space homogeneous kinetic equation modeling the emission, absorption, and scattering of neutrinos on a matter background can be written as (see, e.g., \cite{bruenn_1985,mezzacappaBruenn_1993})
\be\label{tpeqn1d}
\bal
    \partial_t f(x,\mu,\varepsilon,t) = \cC(f)(x,\mu,\varepsilon,t)
    \equiv \mathcal C_{\EmAb}(f) + \mathcal C_{\Iso}(f) + \mathcal C_{\NES}(f,g),
\eal
\ee
where $f\in[0,1]$ is the phase-space distribution function depending on position $x\in D^{x}\subset\bbR$, direction cosine $\mu\in\bbS^{1}=[-1,1]$, energy $\varepsilon\in\bbR^{+}$, and time $t\in\bbR^{+}$, and where $g=1-f$.  
(Since we consider the space homogeneous case in this paper, we will suppress the explicit dependence on the position coordinate $x$ from hereon.)  
On the right-hand side of Eq.~\eqref{tpeqn1d}, the collision operator includes contributions from emission and absorption, isoenergetic scattering, and neutrino--electron scattering (NES), given by
\be\label{collisionterm}
\bal
    \mathcal C_{\EmAb}(f) = & \eta(\varepsilon) - \chi(\varepsilon) f(\mu, \varepsilon), \\
    \mathcal C_{\Iso}(f) = & \int_{\mathbb{S}^1} \sigma(\varepsilon, \mu, \mu')f(\varepsilon, \mu') d\mu' - f(\mu, \varepsilon)\int_{\mathbb{S}^1}\sigma(\varepsilon, \mu, \mu') d\mu',\\
    \mathcal C_{\NES}(f,g) = & g(\mu,\varepsilon)\int_{\mathbb{R}^+}\int_{\mathbb{S}^1} R^{\IN}(\varepsilon, \varepsilon', \mu, \mu')f(\mu',\varepsilon')d\mu'dV_{\varepsilon'} \\
    & -f(\mu,\varepsilon)\int_{\mathbb{R}^+}\int_{\mathbb{S}^1}R^{\OUT}(\varepsilon, \varepsilon', \mu, \mu')g(\mu',\varepsilon')d\mu'dV_{\varepsilon'},
\eal
\ee
respectively. 

In Eq.~\eqref{collisionterm}, $\eta$ is the emissivity, $\chi$ the absorptivity (corrected for stimulated absorption \cite{mezzacappaBruenn_1993}), $\sigma$ the isoenergetic scattering kernel, $R^{\IN/\OUT}$ the NES in- and out-scattering kernels, and $dV_{\varepsilon}=\varepsilon^{2}d\varepsilon$.  
The isoenergetic scattering operator changes the particle direction, but not energy (i.e., couples globally in momentum space angle), and is sometimes used to model neutrino scattering off nucleons and nuclei.  
Since electrons are less massive, the NES operator includes particle direction \emph{and} energy changes (i.e., couples globally in momentum space angle and energy).  
The NES operator is also nonlinear due to the Pauli blocking factors, $g$.  
To reduce the dimensionality of the problem, we have imposed axial symmetries in momentum space in Eq.~\eqref{tpeqn1d}.  
The derivation of Eq.~\eqref{tpeqn1d} from the corresponding equation without imposed symmetries can be found in Appendix~\ref{sec-a}. 
\EE{We need to define $f^{\eq}$: $\cC_{\EmAb}(f^{\eq})=0\to f^{\eq}=\eta/\chi$.  Also, since $f^{\eq}$ is isotropic (independent of $\mu$), $\cC_{\Iso}(f^{\eq})=0$.}
The isoenergetic scattering and NES operators conserve particles, i.e.,
\be\label{ptc}
\bal
    \int_{\bbS^{1}}\cC_{\Iso}(f)d\mu = 0
    \quad\text{and}\quad
    \int_{\bbR^{+}}\int_{\bbS^{1}}\cC_{\NES}(f)d\mu dV_{\varepsilon} = 0,
\eal
\ee
where we have used the in-out invariance of the NES scattering rates \cite{cernohorsky_1994},
$$
R^{\IN}(\varepsilon, \varepsilon', \mu, \mu')=R^{\OUT}(\varepsilon', \varepsilon, \mu', \mu).
$$
The kinetic equation (\ref{tpeqn1d}) is subject to the initial condition 
\be\label{tpinit}
f(\mu,\varepsilon,t=0) = f_0(\mu,\varepsilon).
\ee

We approximate the angular dependence of the isoenergetic scattering kernel $\sigma$ in $\mathcal C_{\Iso}$ with a truncated expansion in orthogonal Legendre polynomials ($\sigma\approx\sigma_{M}$; see Eq.~\eqref{isosigma4}), so that the isoenergetic scattering $\mathcal C_{\Iso}$ is approximated by
\be\label{collisionIso}
\bal
    \mathcal C_{\Iso}^{M}(f) = 4\pi \sum_{\ell=0}^M R_\ell(\varepsilon) P_\ell(\mu)m_\ell(\varepsilon) - 4\pi R_0(\varepsilon)f(\varepsilon, \mu),
\eal
\ee
where we have defined the angular moments
\be\label{faverage}
    m_\ell(\varepsilon,t) = \frac{1}{2}\int_{\bbS^{1}}  P_\ell(\mu) f(\varepsilon,\mu,t)d\mu,
\ee
and where (see Appendix~\ref{sec-b} for details)
\be\label{ReexpISO}
    R_\ell(\varepsilon) = \frac{2\ell+1}{2} \int_{\bbS^{1}} R^{\Iso}(\varepsilon, x)P_\ell(x) dx.
\ee
\begin{assumption}\label{assumRl}
For $R_\ell$ in (\ref{ReexpISO}), we have the following assumptions.
\begin{enumerate}
    \item For $\ell = 0$, we assume
    \be
    \bal
    0< \min_{\varepsilon \in \Omega_\varepsilon} R_0 \leq R_0 \leq \max_{\varepsilon \in \Omega_\varepsilon} R_0.
    \eal
    \ee
    \item For $1\leq \ell \leq M$, there exist constants $R_{\min}$ and $R_{\max}$ such that
\be
0<R_{\min} \leq R_0-\frac{1}{2\ell+1}R_\ell \leq R_{\max}.
\ee
    \item There exists a constant $\sigma_{\min}$ such that
    \be
    \sigma_M (\varepsilon, \mu, \mu') =  2\pi \sum_{l=0}^M R_\ell(\varepsilon) P_\ell(\mu) P_\ell(\mu') \geq \sigma_{\min}>0.
 \ee
\end{enumerate}  
\end{assumption}


Similarly, by expanding the angular dependence of the NES kernels $R^{\IN/\OUT}$ in truncated series of Legendre polynomials, $\cC_{\NES}$ may be approximated as
\be\label{nesleg+}
\bal
    \mathcal{C}_{\NES}^{M}(f,g) 
    = 4\pi g(\mu, \varepsilon)\sum_{\ell=0}^MP_l(\mu) \xi^{\IN,f}_\ell(\varepsilon) - 4\pi f(\varepsilon, \mu)\sum_{\ell=0}^M P_\ell(\mu) \xi^{\OUT,g}_\ell(\varepsilon),
\eal
\ee
where 
\begin{align}
    \xi^{\IN,f}_\ell(\varepsilon)
    &=\int_{\mathbb{R}^+} \Phi_\ell^{\IN}(\varepsilon, \varepsilon') m_\ell(\varepsilon') dV_{\varepsilon'}, \\
    \xi^{\OUT,g}_\ell(\varepsilon)
    &=\int_{\mathbb{R}^+} \Phi_\ell^{\OUT}(\varepsilon, \varepsilon') (\delta_{0\ell}-m_\ell(\varepsilon')) dV_{\varepsilon'},
\end{align}
in which (see Appendix~\ref{sec-b} for details)
\be\label{ReINOUT+}
    \Phi_\ell^{\IN/\OUT}(\varepsilon, \varepsilon') = \frac{2\ell+1}{2} \int_{\bbS^{1}} R^{\IN/\OUT}(\varepsilon,\varepsilon', x)P_\ell(x) dx.
\ee

To explore the dynamic low rank approximation to the solution of Eq.~\eqref{tpeqn1d}, we will investigate algorithms for solving equations with each collision term in Eq.~\eqref{collisionterm} considered separately (using the truncated expansions in Eqs.~\eqref{collisionIso} and \eqref{nesleg+} for isoenergetic scattering and NES, respectively), and with increasing degree of complexity.
More specifically, we consider the following three cases
\begin{enumerate}
    \item Emission and absorption, governed by the linear equation
    \be\label{tp1}
        \partial_t f= \mathcal{C}_{\EmAb}(f).
    \ee
    \item Isoenergetic scattering, governed by the linear equation
    \be\label{tp2}
        \partial_t f= \mathcal{C}_{\Iso}^{M}(f).
    \ee
    It can be verified that the solution conserves the zeroth moment, 
    \be
    m_0(\varepsilon,t) = m_0(\varepsilon,0), \quad \forall t>0,
    \ee
    and conserves the total number of particles, 
    \be
    \int_{\bbR^{+}}\int_{\bbS^{1}} f(\mu,\varepsilon,t) d\mu dV_\varepsilon = \int_{\bbR^{+}}\int_{\bbS^{1}} f_0(\mu,\varepsilon)d\mu dV_\varepsilon, \quad \forall t>0.
    \ee
    Moreover, the solution converges to the equilibrium solution 
    \be
    f \rightarrow f^\teq = m(\varepsilon,0),  \quad t \rightarrow \infty.
    \ee
    \item NES, governed by the nonlinear equation
    \be\label{tp4}
        \partial_t f= \mathcal{C}_{\NES}^{M}(f,1-f).
    \ee
\end{enumerate}

%in a computational domain $\Omega=\Omega_{\mu}\otimes \Omega_{\varepsilon}$ with $\Omega_{\mu}=\mathbb{S}^1=[-1,1]$ and $\Omega_{\varepsilon} \subset \mathbb{R}^+$.

\subsection{DG discretization and matrix equations}

We set the computation domain $\Omega=\Omega_\mu \otimes \Omega_\varepsilon$, where $\Omega_\mu=\mathbb{S}^1$ and $\Omega_\varepsilon \subset \mathbb{R}^+$, we partition the domain  $\Omega$ into computational element 
$$
K_{ij} = \{(\mu, \varepsilon): \mu \in [\mu_{i-1/2}, \mu_{i+1/2}], \ \varepsilon\in [\varepsilon_{j-1/2}, \varepsilon_{j +1/2}] \},
$$
where $1\leq i \leq N_\mu$, and $1\leq j \leq N_\varepsilon$, and it satisfies $\Omega=\cup_{ij}K_{ij}$. We denote the mesh size in each direction by $h_{v}:=\max_i (v_{i+1/2}-v_{i-1/2})$, where $v=\mu, \varepsilon$.

We then define the discontinuous Galerkin finite element space in each direction as
\be\label{dgspace}
V_{v, h} = \{\phi \in L^2(\Omega_v): \phi|_{[v_{l-1/2},v_{l+1/2} ]} \in \cP_{k}([v_{l-1/2},v_{l+1/2} ]), 1\leq l \leq N_v\},
\ee
where $v=\mu, \varepsilon$, and $\cP_{k}$ is polynomials of degree no more than ${k}$.
The discontinuous Galerkin finite element space is defined as
$$
V_h = V_{\mu,h}\otimes V_{\varepsilon,h} = \{v : v|_{K_{ij}} \in \cQ_k(K_{ij}), 1\leq i \leq N_\mu, 1\leq j \leq N_\varepsilon\},
$$
where $\cQ_k$ denotes the space of tensor-product polynomials of degree at most $k$ for each variable defined on $K_{ij}$.

The weighted $L^2$ inner product of two functions $v,w$ in $\Omega$ is denoted by
$$
(v,w;\varepsilon^2)_{\Omega} =(\varepsilon^2v,w)_{\Omega} = \int_{\Omega_\varepsilon} \int_{\Omega_\mu} vw d\mu dV_{\varepsilon} =
 \int_{\Omega_\varepsilon} \int_{\Omega_\mu} vw \varepsilon^2 d\mu d{\varepsilon}.
$$
\EE{Why the weights? Discuss combining the weight with $f$ and discretize $f\varepsilon^{2}$ versus keeping weight separate and discretize $f$.}
Generally, if $v$ is a function, and $\mathcal{V} = [v_1, \cdots, v_{m'}]^T$, $\mathcal{W} = [w_1, \cdots, w_{n'}]^T$ are vector functions on domain $D$, then 
\be
\bal
(v,W;\phi(\varepsilon))_{D} = & (W,v;\phi(\varepsilon))_{D} = [ (v,w_1;\phi(\varepsilon))_{D}, \cdots, (v,w_{n'};\phi(\varepsilon))_{D} ]^T,\\
(V,W^T;\phi(\varepsilon))_{D} = & (W^T, V;\phi(\varepsilon))_{D} = [(v_i,w_j;\phi(\varepsilon))_{D}]_{m'\times n'},
\eal
\ee
where $\phi(\varepsilon) > 0$ be a weighted function.

For Legendre polynomials $P_{\ell}(\mu)$, we denote its piecewise $L^2$ projection onto $V_{\mu, h}$ by $\Pi P_\ell$ satisfying
\be\label{PiPl}
(\Pi P_{\ell}, w_h)_{\mathbb{S}^1} = (P_\ell, w_h)_{\mathbb{S}^1}, \quad \forall w_h \in V_{\mu,h}.
\ee
Then we have that if $0\leq \ell \leq k$, it follows $\Pi P_\ell(\mu)= P_{\ell}(\mu)$; if $k+1 \leq \ell \leq M$, for any given $\tau>0$, we have that when the meshes are refined enough,
\be\label{Plprojerr}
\|P_\ell - \Pi P_\ell\|_{L^2(\mathbb{S}^1)} \leq \sqrt{2}\tau.
\ee
By (\ref{PiPl}) and (\ref{Plprojerr}), we have for any $\ell' \geq 0$,
\be\label{PiPlerr}
\bal
(\Pi P_\ell, \Pi P_{\ell'})_{L^2(\mathbb{S}^1)} = &(\Pi P_\ell, P_{\ell'})_{L^2(\mathbb{S}^1)} =  \frac{2}{2\ell+1}\delta_{\ell \ell'}, \quad 0 \leq \ell \leq k,\\
\left|(\Pi P_\ell, \Pi P_{\ell'})_{L^2(\mathbb{S}^1)}\right| = & \left|(\Pi P_\ell, P_{\ell'})_{L^2(\mathbb{S}^1)}\right|  \leq  \frac{2}{2\ell+1}\delta_{\ell \ell'} + 2\tau, \quad  k+1 \leq \ell \leq M,
\eal
\ee
where $\delta_{\ell\ell'}$ is a Kronecker delta function.

\subsubsection{The semi-discrete full rank DG scheme}

The semi-discrete DG schemes for equations (\ref{tp1}-\ref{tp4}) are to find $f_{h}(t)\in V_h$ such that
\be\label{semiDG}
(\partial_t f_h, w_h;\varepsilon^2)_{\Omega} = \mathcal{A}(f_h, w_h), \quad \forall w_h \in V_h,
\ee
where the bilinear functional for equation (\ref{tp1}), 
\be\label{bifs1}
\bal
\mathcal{A}(f_h, w_h)  = & \mathcal{A}_{\EmAb}(f_h,w_h) :=  (C_{\EmAb}(f_h,g_h),w_h;\varepsilon^2)_{\Omega}\\
= & \left(\varepsilon^2\eta(\varepsilon), w_h\right)_{\Omega}-\left(\varepsilon^2\chi(\varepsilon) f_h(\mu, \varepsilon), w_h\right)_{\Omega};
\eal
\ee
for equation (\ref{tp2}),
\be\label{bifs2}
\bal
\mathcal{A}(f_h, w_h)= & \mathcal{A}_{\Iso}(f_h,w_h):= (C_{\Iso}(f_h,g_h),w_h;\varepsilon^2)_{\Omega}\\
%= &  4\pi \sum_{l=0}^M \left(\varepsilon^2R_l(\varepsilon) P_l(\mu)m_{\ell h}(\varepsilon), w_h\right)_{\Omega}-\left(4\pi \varepsilon^2R_0(\varepsilon)f_h(\varepsilon, \mu), w_h\right)_{\Omega}\\
= & 4\pi \sum_{l=0}^M \left(\varepsilon^2R_l(\varepsilon) \Pi P_l(\mu)m_{\ell h}(\varepsilon), w_h\right)_{\Omega}-\left(4\pi \varepsilon^2R_0(\varepsilon)f_h(\varepsilon, \mu), w_h\right)_{\Omega},
\eal
\ee
where the discretized angular moments is given by
\be
m_{\ell h} = \frac{1}{2}\int_{\bbS^{1}}  \Pi P_\ell(\mu) f_h(\varepsilon,\mu)d\mu,
\ee
and the second equality has used (\ref{PiPl}) since $w_h \in V_h$ is separable.
for equation (\ref{tp4}),
\be\label{bifs4}
\bal
\mathcal{A}(f_h,w_h)= & \mathcal{A}_{\NES}(f_h,w_h):=  (C_{\NES}(f_h,1-f_h),w_h;\varepsilon^2)_{\Omega} \\
=& 4\pi \sum_{l=0}^M \left(\varepsilon^2P_l(\mu) \xi^{\text{IN},f_h}_l(\varepsilon), w_h\right)_{\Omega}-  \left(4\pi \varepsilon^2\xi^{\text{OUT},1}_0(\varepsilon)f_h(\varepsilon, \mu), w_h\right)_{\Omega} \\
& -\left(4\pi \varepsilon^2 f(\mu, \varepsilon)\sum_{l=0}^MP_l(\mu) \left( \xi^{\text{IN},f_h}_l(\varepsilon) -  \xi^{\text{OUT},f_h}_l(\varepsilon) \right), w_h\right)_{\Omega}.
\eal
\ee

The initial data is taken as the weighted piecewise $L^2$ projection of $f_0(\mu,\varepsilon)$, that is 
to find $f_h(0) \in V_h$ such that 
\be\label{semidginit}
(f_h(0),v,w_h;\varepsilon^2)_{\Omega} = (f_0,v,w_h;\varepsilon^2)_{\Omega}, \quad \forall w_h \in V_h.
\ee

It is easy to verify solutions of the semi-discrete DG scheme (\ref{semiDG}) for equation (\ref{tp1}) and (\ref{tp2}) are $L^2$ stable.

\subsubsection{The formulation of the full rank matrix equation}
To explore the low-rank feature of the solutions, we express the functions in the DG finite element space $V_h$ in matrix form. 
Let $\{u_i(\mu)\}_{i=1}^m$, $\{e_j(\varepsilon)\}_{j=1}^n$ be the orthonormal basis functions in DG finite element spaces $V_{\mu,h}$ and $V_{\varepsilon,h}$, respectively.
Here, $m=(k+1)N_\mu$ and $n=(k+1)N_\varepsilon$.
For $f_h(t, \mu, \varepsilon) \in V_h$, it has an expansion
\be\label{DGtoMatDef}
f_h(t, \mu, \varepsilon)= \sum_{i=1}^m \sum_{j=1}^n F_{ij}(t) u_i(\mu) e_j(\varepsilon) = X^T(\mu)F(t)Y(\varepsilon),
\ee
where
\be\label{muepbasis}
X(\mu) = [u_1(\mu), \cdots, u_m(\mu)]^T, \quad Y(\varepsilon)=[e_1(\varepsilon), \cdots, e_n(\varepsilon) ]^T,
\ee
and the coefficient $F_{ij}$ is the entry of the coefficient matrix $F \in \mathbb{R}^{m\times n}$, for each $i$, it solves the linear system
\be
\sum_{j=1}^n F_{ij}(e_j, e_{j'}; \varepsilon^2)_{\Omega_\varepsilon} = (f_h, u_ie_{j'}; \varepsilon^2)_{\Omega}, \quad j' = 1, \cdots, n.
\ee

For given matrices $A,B \in \mathbb{R}^{m'\times n'}$, we denote the Frobenius inner product by
\be\label{frobdef}
(A,B)_\mathcal{F}=\text{tr}(A^TB) =\sum_{i=1}^{m'} \sum_{j=1}^{n'} a_{ij}b_{ij},
\ee
where $a_{ij}$, $b_{ij}$ are the entries of matrices $A,B$, respectively. The Frobenius norm is given by
$$
\|A\|_\mathcal{F} = \sqrt{( A,A)_\mathcal{F}}= \left(\sum_{i=1}^{m'} \sum_{j=1}^{n'} |a_{ij}|^2\right)^{\frac{1}{2}}.
$$
If $A$, $B$ are vectors, the Frobenius inner product and the Frobenius norm degenerate to the regular the inner product of two vectors denoted by $(A,B)$, and the norm of a vector denoted by $\|A\|$.

\begin{definition}\label{SepDef}
A bilinear form $\mathcal{B}(\cdot, \cdot)$ on $V_h\times V_h$ is separable in terms of the basis $\{u_ie_j\}$, $1\leq i \leq m$, $1\leq j \leq n$, if there exists two bilinear forms $\mathcal{B}_\mu:V_{\mu,h}\times V_{\mu,h}\to\R$ and $\mathcal{B}_\varepsilon:V_{\varepsilon,h}\times V_{\varepsilon,h}\to\R$ such that
\be\label{Bsep}
\mathcal{B}(u_{i'}e_{j'},u_ie_j) = \mathcal{B}_\mu(u_{i'},u_i)\mathcal{B}_\varepsilon(e_{j'},e_j),
\ee
where $1\leq i' \leq m$, $1\leq j' \leq n$.
\end{definition}
\begin{definition}\label{SepDefL}
A linear form $\mathcal{L}(\cdot)$ on $V_h$ is separable in terms of the basis $\{u_ie_j\}$, $1\leq i \leq m$, $1\leq j \leq n$, if there exists two linear forms $\mathcal{L}_\mu:V_{\mu,h}\to\R$ and $\mathcal{L}_\varepsilon:V_{\varepsilon,h}\to\R$ such that
\be\label{Lsep}
\mathcal{L}(u_ie_j) = \mathcal{L}_\mu(u_i)\mathcal{L}_\varepsilon(e_j).
\ee
\end{definition}

\begin{proposition}\label{prop2.1}
Suppose $\mathcal{B}(\cdot, \cdot)$ is a separable bilinear form on $V_h\times V_h$ satisfying (\ref{Bsep}).
Let $z_h, w_h \in V_h$, and  and $Z, W \in \mathbb{R}^{m\times n}$ be the coefficient matrices of $z_h, w_h$, respectively, then it follows
\[
\mathcal{B}(z_h,w_h) = (B_\mu ZB_\varepsilon^T,W)_\mathcal{F},
\]
where $B_\mu\in\R^{m\times m}$ and $B_\varepsilon\in\R^{n\times n}$ are the stiffness matrices in terms of the bases $\{u_i\}$ and $\{e_j\}$ with the entries given by
\[
(B_\mu)_{ii'} = \mathcal{B}_\mu(u_{i'},u_i), \quad (B_\varepsilon)_{jj'} = \mathcal{B}_\varepsilon(e_{j'},e_j).
\]
\end{proposition}
\begin{proof}
By assumption, we have
\bes
\bal
\mathcal{B}(z_h,w_h) &= \mathcal{B}\left(\sum_{i'j'} Z_{i'j'} u_{i'} e_{j'}, \sum_{ij} W_{ij} u_i e_j \right) 
=\sum_{i'j'}\sum_{ij} Z_{i'j'}W_{ij}\mathcal{B}_\mu(u_{i'},u_i)\mathcal{B}_\varepsilon(e_{j'},e_j) \\
= & \sum_{i'j'}\sum_{ij} Z_{i'j'}W_{ij} (B_\mu)_{ii'}(B_\varepsilon)_{jj'} 
=\sum_{ij} \left(\sum_{i'j'} (B_\mu)_{ii'} Z_{i'j'} (B_\varepsilon^T)_{j'j} \right) W_{ij} \\
=&  \sum_{ij} (B_\mu Z B_\varepsilon^T)_{ij}W_{ij} = (B_\mu ZB_\varepsilon^T,W)_\mathcal{F}.
\eal
\ees
Thus, the conclusion holds.  
\end{proof}

\begin{proposition}\label{prop2.2} 
Suppose $\mathcal{L}(\cdot)$ is a separable linear form on $V_h$ satisfying (\ref{Lsep}).
Let $w_h \in V_h$ given by (\ref{DGtoMatDef}), then we have
\be\label{lwdecomp}
\mathcal{L}(w_h) = L_\mu^T W L_\varepsilon=(L_\mu L_\varepsilon^T,W)_\mathcal{F},
\ee
where $L_\mu\in\R^{m}$ and $L_\varepsilon\in\R^{n}$ are vectors in terms of the bases $\{u_i\}$ and $\{e_j\}$ with the entries given by
\[
(L_\mu)_{i} = \mathcal{L}_\mu(u_i), \quad (L_\varepsilon)_{j} = \mathcal{L}_\varepsilon(e_j).
\]
\end{proposition}
\begin{proof}
By assumption, we have
\bes
\bal
\mathcal{L}(w_h) &= \mathcal{L}\left(\sum_{ij} W_{ij} u_i e_j \right) 
=\sum_{ij}W_{ij}\mathcal{L}_\mu(u_i)\mathcal{L}_\varepsilon(e_j) = \sum_{ij} W_{ij} (L_\mu)_{i}(L_\varepsilon)_{j} \\
=&  \sum_{ij} (L_\mu L_\varepsilon^T)_{ij}w_{ij} = L_\mu^T W L_\varepsilon= (L_\mu ,WL_\varepsilon)_\mathcal{F}= (L_\mu L_\varepsilon^T,W)_\mathcal{F}.
\eal
\ees
Thus, the conclusion holds.  
\end{proof}

\begin{remark}
Note that $L_\mu L_\varepsilon^T$ in (\ref{lwdecomp}) is a rank-$1$ matrix, and one doesn't need to evaluate the multiplication directly. In low rank approximation, it is usually replaced by an equivalent form
\be
L_\mu L_\varepsilon^T = USE^T,
\ee
where $U\in \mathbb{R}^{m\times 1}$, $S\in \mathbb{R}^{1\times 1}$, and $E\in \mathbb{R}^{n\times 1}$.
\end{remark}

\begin{corollary}\label{bilform}
For a given function $\phi(\varepsilon)>0$, the bilinear form $(\cdot, \cdot; \phi(\varepsilon))_{\Omega}$ is separable with respect to the basis $\{e_iu_j\}$, $1\leq i \leq m$, $1\leq j \leq n$. 
Let $z_h, w_h \in V_h$, and $Z, W \in \mathbb{R}^{m\times n}$ be the coefficient matrices of $z_h, w_h$, respectively, then it follows that
\be\label{L2Mat}
(z_h,w_h;\phi(\varepsilon))_{\Omega} = (Z  B_{\varepsilon}, W)_\mathcal{F},
\ee
where the symmetric positive-definite block matrix
\be\label{dllp}
(B_{\varepsilon})_{n\times n}=(\phi(\varepsilon)Y^T(\varepsilon), Y(\varepsilon))_{\Omega_\varepsilon}.
\ee
Namely, for any matrix $W\in \mathbb{R}^{m\times n}$, it follows
\be\label{L2Mat0}
(W B_{\varepsilon}, W)_\mathcal{F} \geq 0,
\ee
the equality holds only if $W=0$. Moreover, there exists a upper block matrix $C_\varepsilon$ such that
\be\label{Adecom}
B_\varepsilon = C_\varepsilon^T C_\varepsilon.
\ee
\end{corollary}
\begin{proof}
With the given basis $\{e_iu_j\}$, we have
\bes
\bal
(u_ie_j,u_{i'}e_{j'};\phi(\varepsilon))_{\Omega}  = (u_i,u_{i'})_{\Omega_\mu}(e_j,e_{j'};\phi(\varepsilon))_{\Omega_\varepsilon}= (u_i,u_{i'})_{\Omega_\mu}(e_j,e_{j'};\phi(\varepsilon))_{\Omega_\varepsilon},
\eal
\ees
so the the bilinear form $(\cdot, \cdot; \phi(\varepsilon))_{\Omega}$ on $V_h\times V_h$
is separable by the Definition \ref{SepDef}. Then by Proposition \ref{prop2.1}, it follows
$$
(z_h,w_h;\phi(\varepsilon))_{\Omega} = (B_\mu Z B_{\varepsilon}^T, W)_\mathcal{F},
$$
where $(B_{\mu})_{ii'}=(u_{i'},u_i)_{\Omega_{\mu}}$, $(B_{\varepsilon})_{jj'}=(e_{j'},e_j;v(\varepsilon))_{\Omega_\varepsilon}$.
Since $\{u_i(\mu)\}_{i=1}^m$, $\{e_j(\varepsilon)\}_{j=1}^n$ are the orthonormal basis functions, so we have
$B_{\mu}=I_{m}$ with $I_m$ being the identity matrix, and $(B_{\varepsilon})_{n\times n}$ being given by (\ref{dllp}).
%and $(A_{\varepsilon})_{n\times n}=\text{diag} \{\bar D_1, \cdots, \bar D_{N_{\varepsilon}}\}$, where $I$ is an identity matrix, and $D_\nu\in \mathbb{R}^{(k+1)\times(k+1)}$, $l=1,\cdots, N_{\varepsilon}$ with $(D_\nu)_{ll'}$ given by (\ref{dllp}).
Let $w_h \in V_h$ with $W$ being the coefficient matrix, then we have
\be
\bal
(W B_{\varepsilon}, W)_\mathcal{F} = (w_h,w_h;\phi(\varepsilon))_{\Omega}=\|\sqrt{\phi(\varepsilon)}w_h\|^2_{L^2(\Omega)} \geq 0,
\eal
\ee
which indicates that the matrix $B_\varepsilon$ is a positive-definite matrix. By the Cholesky decomposition, the decomposition (\ref{Adecom}) holds.
\end{proof}

We denote the vectors
\be\label{Lmuvec}
L_{\ell} = (P_\ell(\mu), X(\mu))_{\Omega_\mu}= (\Pi P_\ell(\mu), X(\mu))_{\Omega_\mu} \in \mathbb{R}^{m\times 1},
\ee
where $P_\ell(\mu)$ are the Legendre polynomials, and $X(\mu)$ is the orthonormal basis given in (\ref{muepbasis}), then by Lemma \ref{basisproperty}, it follows for any $\ell' \geq 0$,
\be\label{Lmulprop}
\bal
L_{\ell}^T L_{\ell'} = & \frac{2}{2\ell+1} \delta_{\ell\ell'}, \quad  0\leq \ell \leq k, \\
L_{\ell}^T L_{\ell'} = & (\Pi P_\ell(x), P_{\ell'}(x))_{S_1}, \quad \ell \geq k+1,
\eal
\ee
where $\delta_{\ell\ell'}$ is a Kronecker delta function.

By Proposition \ref{prop2.1} and Corollary \ref{bilform}, the bilinear form $\mathcal{A}_{\EmAb}(f_h,w_h)$ in (\ref{bifs1}) is separable, and it follows
\be\label{Aealinear}
\mathcal{A}_{\EmAb}(f_h,w_h) = \left( L_{0} (L^{\EmAb})^T-F A^{\EmAb}, W \right)_\mathcal{F},
\ee
where $L_{0} = (1, X(\mu))_{\Omega_\mu} \in \mathbb{R}^{m \times 1}$, $L^{\EmAb}  =(\varepsilon^2\eta(\varepsilon), Y(\varepsilon))_{\Omega_\varepsilon} \in \mathbb{R}^{n\times 1}$, and the positive definite symmetric block matrix
\be\label{AeEA}
A^{\EmAb}=\left(\varepsilon^2\chi(\varepsilon) Y(\varepsilon), Y^T(\varepsilon) \right)_{\Omega_\varepsilon} \in \mathbb{R}^{n\times n}.
\ee 
By Corollary \ref{bilform}, there exists a upper block matrix $C^\EmAb$ such that
\be\label{Aedecomp}
A^\EmAb = (C^\EmAb)^TC^\EmAb.
\ee

Similarly, the bilinear functional $\mathcal{A}_{\Iso}(f_h,w_h)$ in (\ref{bifs2}) is separable, and it follows
\be\label{isomat}
\bal
\mathcal{A}_{\Iso}(f_h,w_h) 
= &  \left(2\pi \sum_{\ell=0}^M L_{\ell} L_{\ell}^T F A^{\Iso}_\ell-4\pi F A^{\Iso}_0, W \right)_\mathcal{F}
\eal
\ee
where $L_{\ell} \in \mathbb{R}^{m\times 1}$ given by (\ref{Lmuvec}), and the symmetric block matrices
\be\label{AeIso}
A^{\Iso}_\ell= \left(\varepsilon^2R_\ell(\varepsilon) Y(\varepsilon), Y^T(\varepsilon) \right)_{\Omega_\varepsilon} \in \mathbb{R}^{n\times n}.
\ee
In addition, the $\ell$th moment of $f_h$ is given by
\be\label{fhexpress}
m_\ell(\varepsilon) =  \frac{1}{2}\int_{\Omega_\mu}P_\ell(\mu) f_h(\mu,\varepsilon)d\mu = \frac{1}{2} \left(\int_{\Omega_\mu}P_l(\mu) X^T(\mu) d\mu \right) F Y(\varepsilon) = \frac{1}{2} L_\ell^T F Y(\varepsilon).
\ee
Let $f_h$ be the solution of the semi-discrete DG scheme (\ref{semiDG}), then the coefficient matrix $F$ satisfies the following matrix differential equation
\be\label{semidgmat}
\partial_t F(t) A_\varepsilon = G(F(t)),
\ee
in which we have for (\ref{tp1}),
\be\label{Gformula1}
\bal
G(F)=& G_1(F)=
L_{0} (L^{\EmAb})^T - F A^{\EmAb},
\eal
\ee
for (\ref{tp2}),
\be\label{Gformula2}
\bal
G(F)=& G_2(F) = 2\pi \sum_{\ell=0}^M L_{\ell} L_{\ell}^T F A^{\Iso}_\ell -4\pi F A^{\Iso}_{\varepsilon,0}.
\eal
\ee
Here, the positive-definite symmetric block matrix 
\be\label{Avare}
A_\varepsilon= \left(\varepsilon^2 Y(\varepsilon), Y^T(\varepsilon) \right)_{\Omega_\varepsilon} \in \mathbb{R}^{n\times n}.
\ee
By Corollary \ref{bilform}, there exists a upper block matrix $C_\varepsilon$ such that
\be\label{Adecomp}
A_{\varepsilon} = (C_{\varepsilon})^TC_{\varepsilon}.
\ee
%satisfying
%\be\label{AepP}
%(WA_\varepsilon, W)_{\cF} \geq 0, \quad \forall W\in \bbR^{m\times n},
%\ee
%and equality holds only if $W=0$.
The initial coefficient matrix $F(0)$ is obtained by solving (\ref{semidginit}).

\subsubsection{First order fully-discrete full rank DG schemes}
Here we apply an appropriate time discretization to the semi-discrete DG scheme given by Eq.~\eqref{semiDG}, for each of the cases given by Eqs.~\eqref{bifs1}-\eqref{bifs4}.  
The corresponding matrix equation can be obtained by applying the same type of time discretization to the matrix differential equation in Eq.~\eqref{semidgmat}.
For simplicity, we denote 
\be
    D_t v^{\mathfrak{n}+1}
    = \frac{v^{\mathfrak{n}+1}-v^\mathfrak{n}}{\Delta t},
\ee
where $v$ can be any function or matrix.

We wish to use implicit time discretization methods because short time scales induced by the collision operators can render explicit methods inefficient.  
Let $f_h^\mathfrak{n}$ denote the approximation to $f_h(t_\mathfrak{n},\mu,\varepsilon)$, where $t_\mathfrak{n}=\mathfrak{n}\Delta t$ with $\Delta t$ being the time step.
Then, with backward Euler time discretization, the first order, fully discrete DG scheme for Eqs.~\eqref{tp1}-\eqref{tp2} is then to find $f_h^\mathfrak{n+1} \in V_h$ such that,
\be\label{fullDG1}
    \left(D_t f_h^{\mathfrak{n}+1}, w_h;\varepsilon^2 \right)_{\Omega} = \mathcal{A}(f_h^{\mathfrak{n}+1},w_h), \quad \forall w_h \in V_h,
\ee
where $\mathcal{A}(\cdot, \cdot)$ for equation (\ref{tp1}) is given by Eq.~\eqref{bifs1}, and for equation (\ref{tp2}) is given by
\be\label{bifs2+}
\bal
%\mathcal{A}(f_h^{\mathfrak{n}+1}, w_h)= 
\mathcal{A}_{\Iso}(f_h^{\mathfrak{n}+1},w_h)= 4\pi \sum_{l=0}^M \left(\varepsilon^2R_l(\varepsilon) \Pi P_l(\mu)m_{\ell h}^{\mathfrak{n}+1}(\varepsilon), w_h\right)_{\Omega}-\left(4\pi \varepsilon^2R_0(\varepsilon)f_h^{\mathfrak{n}+1}(\varepsilon, \mu), w_h\right)_{\Omega},
\eal
\ee
and the angular moments
\be
m_{\ell h}^{\mathfrak{n}+1} = \frac{1}{2}\int_{\bbS^{1}}  \Pi P_\ell(\mu) f_h^{\mathfrak{n}+1}(\varepsilon,\mu)d\mu,
\ee

Below we list some results regarding the fully discrete scheme in Eq.~\eqref{fullDG1}, using either the bilinear for in Eq.~\eqref{bifs1} or Eq.~\eqref{bifs2}.  
(The proofs are straightforward and have been omitted.)  
Later, we wish to prove corresponding results in the low-rank setting.  

We denote by $f_h^{\text{eq}} = X(\mu) F^{\text{eq}} Y(\varepsilon)$ the piecewise weighted $L^2$ the projection of the equilibrium solution $f^{\text{eq}}(\varepsilon)$ for the problem (\ref{tp1}) into the DG space $V_h$ satisfying
\be\label{feql2proj}
    \mathcal{A}_\EmAb(f_h^{\text{eq}}, w_h) = 0, \quad \forall w_h \in V_h,
\ee
then we have
\be\label{Feqmat}
    F^{\text{eq}}=L_{0}(L^{{\EmAb}})^T(A^\EmAb)^{-1}.
\ee

\begin{proposition}\label{fullDG1lem}
The full rank DG scheme (\ref{fullDG1}) for problem (\ref{tp1}) admits a unique solution $f_h^\mathfrak{n} \in V_h$. Moreover, we have the following results.
\begin{itemize}
    \item[(1).] The solution is uniformly bounded,
\be\label{emabfullstab}
\bal
\|\varepsilon f_h^{\mathfrak{n}}\|_{L^2(\Omega)} \leq c^\mathfrak{n} \|\varepsilon f_{0}\|_{L^2(\Omega)} + \frac{1}{\min_{\varepsilon \in \Omega_\varepsilon}\chi} (1-c^\mathfrak{n})\|\varepsilon\eta\|_{L^2(\Omega)},
\eal
\ee
where
\be\label{ratior}
c = \frac{1}{1+\Delta t \min_{\varepsilon \in \Omega_\varepsilon} \chi (\varepsilon)}.
\ee
\item[(2).] Let $f^{\text{eq}}_h$ be the piecewise $L^2$ projection of the equilibrium solution $f^{\text{eq}}$ in (\ref{feql2proj}) for problem (\ref{tp1}), then it follows
\be\label{Lstab}
\bal
\|\varepsilon (f_h^{\mathfrak{n}} - f_h^{\text{eq}})\|_{L^2(\Omega)} \leq & c^\mathfrak{n} \|\varepsilon (f_h^{0} - f_h^\teq) \|_{L^2(\Omega)}.
%+\frac{1}{\min_{\varepsilon \in \Omega_\varepsilon}\chi} (1-c^\mathfrak{n})\|\varepsilon{\chi}(f^{\text{eq}}- f_h^{\text{eq}})\|_{L^2(\Omega)}.
\eal
\ee
%where $c$ is given by (\ref{ratior}).
\end{itemize}

\end{proposition}

\iffalse
\begin{remark}
We can further simply the last term in (\ref{Lstab}) by applying the following identity that any $v(\varepsilon)$ it holds
\be
\|v\|_{L^2(\Omega)}  = |\Omega_\mu|^{\frac{1}{2}}\|v\|_{L^(\Omega_\varepsilon)} = \sqrt{2}\|v\|_{L^2(\Omega_\varepsilon)}. 
\ee
\end{remark}
\fi

By Assumption \ref{assumRl}, (\ref{PiPl}) and (\ref{PiPlerr}), as the meshes are refined sufficiently, we further have the following results.
 \begin{itemize}
    \item[(1).] For $1\leq \ell \leq M$, there exists $0<R'_{\min} \leq \min\{ R_{\min}, \min_{\varepsilon \in \Omega_\varepsilon} R_0 (\varepsilon)\}$ and $R'_{\max}$ such that
\be\label{assumRlp}
R'_{\min} \leq R_0-\frac{1}{2}\|\Pi P_\ell\|_{L^2(\mathbb{S}^1)} R_\ell \leq R'_{\max}.
\ee
    \item[(2).] There exists $\sigma'_{\min}>0$ such that 
    \be\label{sigmamh}
    \sigma_{M,h} (\varepsilon, \mu, \mu') =  2\pi \sum_{l=0}^M R_\ell(\varepsilon) \Pi P_\ell(\mu) \Pi P_\ell(\mu') \geq \sigma'_{\min}>0.
 \ee
\end{itemize} 

\begin{proposition}\label{fullDG2lem}
The full rank DG scheme (\ref{fullDG1}) for problem (\ref{tp2}) admits a unique solution. In addition, we have the following results.
\begin{itemize}
    \item[(1).] The weighted $L^{2}$ stability holds in the following sense
\be\label{isol2stab}
\bal
\|\varepsilon f_h^{\mathfrak{n}+1}\|^2_{L^2(\Omega)} = & \|\varepsilon f_h^{\mathfrak{n}}\|^2_{L^2(\Omega)} - \|\varepsilon(f_h^{\mathfrak{n}+1}-f_h^{\mathfrak{n}})\|^2_{L^2(\Omega)} \\
& - \Delta t \int_{\Omega_\varepsilon}\varepsilon^2\int_{\Omega_\mu}\int_{\Omega_{\mu'}} \sigma_{M,h}(\varepsilon, \mu, \mu') \left(f^{\mathfrak{n}+1}_h(\varepsilon,\mu) -  f^{\mathfrak{n}+1}_h(\varepsilon, \mu') \right)^2 d\mu'd\mu d\varepsilon.
\eal
\ee
\item[(2).] 
The solution conserves the zeroth moment
\be
m_{0h}^\mathfrak{n} = m_{0h}^0, \quad \forall \mathfrak{n}.
\ee
Therefore, it conserves the total number of particles, namely,
\be\label{isopartcons}
\int_{\Omega_\varepsilon}\int_{\Omega_\mu} f_h^\mathfrak{n} d\mu dV_{\varepsilon} = 2\int_{\Omega_\varepsilon} m_{0h}^\mathfrak{n} dV_{\varepsilon} = 2\int_{\Omega_\varepsilon} m_{0h}^0 dV_{\varepsilon} =\int_{\Omega_\varepsilon}\int_{\Omega_\mu} f_h^0 d\mu dV_{\varepsilon}, \quad \forall \mathfrak{n}.
\ee
\item[(3).] As the meshes are refined sufficiently, the solution converges to the $0$th initial moment $m_{0h}^0$ in the following convergence rate,
\be\label{ffeqbdd0}
\bal
\|\varepsilon ( f_h^{\mathfrak{n}} - m_{0h}^0 )\|_{L^2(\Omega)} \leq  c^\mathfrak{n} \|\varepsilon ( f_h^{0} - m_{0h}^0 )\|_{L^2(\Omega)},
\eal
\ee
where the parameter
\be\label{ratioriso}
c = \frac{\alpha}{1+ 2\pi\Delta t R'_{\min} },
\ee
and the constant $\alpha$ depends on $M$, $R'_{\min}$.
\end{itemize}
\end{proposition}
\begin{proof}
We prove (3) only. We take $w_h = \Pi P_\ell(\mu) w_\varepsilon$ in (\ref{fullDG1}) for any $w_\varepsilon \in V_{\varepsilon,h}$, then we have
\be
\bal
& (m_{\ell h}^{\mathfrak{n}+1}-m_{\ell h}^{\mathfrak{n}}, w_\varepsilon; \varepsilon^2)_{\Omega_\varepsilon} =   4\pi\Delta t\left(\left(\frac{1}{2\ell+1}R_\ell-R_0\right) m_{\ell h}^{\mathfrak{n}+1} , w_\varepsilon; \varepsilon^2 \right)_{\Omega_\varepsilon}, \quad 0\leq \ell \leq k,\\
& (m_{\ell h}^{\mathfrak{n}+1}-m_{\ell h}^{\mathfrak{n}}, w_\varepsilon; \varepsilon^2)_{\Omega_\varepsilon} =   4\pi\Delta t \left( \left(\frac{1}{2} \|\Pi P_\ell\|_{L^2(\mathbb{S}^1)}^2R_\ell-R_0\right) m_{\ell h}^{\mathfrak{n}+1} , w_\varepsilon; \varepsilon^2 \right)_{\Omega_\varepsilon} \\
& +4\pi\Delta t \left( \sum_{\ell'=k+1, \ell' \not=\ell}^M \left(\frac{1}{2} (\Pi P_\ell, \Pi P_\ell')_{L^2(\mathbb{S}^1)}R_\ell\right) m_{\ell' h}^{\mathfrak{n}+1} , w_\varepsilon; \varepsilon^2 \right)_{\Omega_\varepsilon}, \quad k+1 \leq \ell \leq M.
\eal
\ee
By taking $w_\varepsilon = m_{\ell h}^{\mathfrak{n}+1}$, we have for $\ell =0$,
\be\label{consmoment}
m_{0 h}^{\mathfrak{n}+1}= m_{0 h}^{\mathfrak{n}}= \cdots = m_{0 h}^{0}; 
\ee
for $1\leq \ell \leq k$,
\be\label{mpmn1bdd}
\|\varepsilon m_{\ell h}^{\mathfrak{n}+1} \|_{L^2(\Omega_\varepsilon)} \leq \frac{1}{1+ 4\pi\Delta t R_{\min} } \|\varepsilon m_{\ell h}^{\mathfrak{n}} \|_{L^2(\Omega_\varepsilon)},
\ee
and for $k+1 \leq \ell \leq M$, by applying (\ref{PiPlerr}) we have
\be\label{momlgk}
\left( 1+ 4\pi\Delta t R'_{\min} \right)\|\varepsilon m_{\ell h}^{\mathfrak{n}+1} \|_{L^2(\Omega_\varepsilon)} \leq \|\varepsilon m_{\ell h}^{\mathfrak{n}} \|_{L^2(\Omega_\varepsilon)} + 4\pi\Delta t \tau \max_{k+1\leq \ell \leq M}\|R_l\|_{L^\infty(\Omega_\varepsilon)}  \sum_{\ell' = k+1, \ell' \not=\ell}^M \|\varepsilon m_{\ell' h}^{\mathfrak{n}+1} \|_{L^2(\Omega_\varepsilon)}.
\ee
As the meshes are refined such that $\tau \leq \frac{R'_{\min}}{2(M-k) \max_{k+1\leq \ell \leq M}\|R_l\|_{L^\infty(\Omega_\varepsilon)} }$, then the summation of (\ref{momlgk}) over $k+1 \leq \ell \leq M$ gives
\be\label{mpmn1bdd1}
\sum_{\ell=k+1}^M \|\varepsilon m_{\ell h}^{\mathfrak{n}+1} \|_{L^2(\Omega_\varepsilon)} \leq  c' \sum_{\ell=k+1}^M\|\varepsilon m_{\ell h}^{\mathfrak{n}} \|_{L^2(\Omega_\varepsilon)},
\ee
where $c'$ is given by (\ref{ratioriso}).
Note that
\be\label{momlfm}
\bal
\|\varepsilon m_{\ell h}^{\mathfrak{n}} \|_{L^2(\Omega_\varepsilon)}^2 = &  \int_{\Omega_\varepsilon} (m_{\ell h}^{\mathfrak{n}})^2 dV_\varepsilon =\frac{1}{4}\int_{\Omega_\varepsilon} \left(\int_{\Omega_\mu} f_h^\mathfrak{n} \Pi P_\ell d\mu \right)^2 dV_\varepsilon \\
= & \frac{1}{4} \int_{\Omega_\varepsilon} \left(\int_{\Omega_\mu} (f_h^\mathfrak{n} - m_{0h}^0) \Pi P_\ell d\mu \right)^2 dV_\varepsilon \leq \frac{1}{4}\|\Pi P_\ell\|_{L^2(\Omega_\mu)}^2 \|\varepsilon(f_h^\mathfrak{n} - m_{0h}^0)\|_{L^2(\Omega)}^2.
\eal
\ee
Thus, (\ref{mpmn1bdd}), (\ref{mpmn1bdd1}) and (\ref{momlfm}) imply that 
\be
\sum_{\ell=1}^M \|\varepsilon m_{\ell h}^{\mathfrak{n}+1} \|_{L^2(\Omega_\varepsilon)} \leq \frac{1}{2} c' \|\varepsilon(f_h^\mathfrak{n} - m_{0h}^0)\|_{L^2(\Omega)} \sum_{\ell=1}^M  \|\Pi P_\ell\|_{L^2(\Omega_\mu)} .
\ee
By (\ref{consmoment}), we can rewrite (\ref{fullDG1}) as
\be\label{frdgre}
\bal
\left((1+4\pi\Delta t R_0)f_h^{\mathfrak{n}+1}, w_h;\varepsilon^2 \right)_{\Omega} = &  \left( f_h^{\mathfrak{n}}+4\pi\Delta t R_0 m_{0h}^0, w_h; \varepsilon^2\right)_{\Omega} \\
& + 4\pi \Delta t \sum_{l=1}^M \left(\varepsilon^2R_l(\varepsilon) \Pi P_l(\mu)m_{\ell h}^{\mathfrak{n}+1}(\varepsilon), w_h\right)_{\Omega}.
\eal
\ee
Subtract $ \left((1+4\pi\Delta t R_0)m_{0h}^0, w_h;\varepsilon^2 \right)_{\Omega} $ from (\ref{frdgre}) and set $w_h =f_h^{\mathfrak{n}+1} - m_{0h}^0 $, we obtain
\be\label{ffeqbdd}
\bal
\|\varepsilon ( f_h^{\mathfrak{n}+1} - m_{0h}^0 )\|_{L^2(\Omega)} \leq  &  c' \|\varepsilon ( f_h^{\mathfrak{n}} - m_{0h}^0 )\|_{L^2(\Omega)}  +4\pi c'\Delta t  \sum_{\ell=1}^M \|R_\ell\|_{L^\infty(\Omega_\varepsilon)}\|\Pi P_\ell\|_{L^2(\Omega_\mu)}\|\varepsilon m_{\ell h}^{\mathfrak{n}+1}\|_{L^2(\Omega_\varepsilon)}\\
\leq & c' \|\varepsilon ( f_h^{\mathfrak{n}} - m_{0h}^0 )\|_{L^2(\Omega)}  +4\sqrt{2}\pi c' \Delta t \max_{\ell} \|R_\ell\|_{L^\infty(\Omega_\varepsilon)} \sum_{\ell=1}^M \|\varepsilon m_{\ell h}^{\mathfrak{n}+1} \|_{L^2(\Omega_\varepsilon)}\\
\leq & c \|\varepsilon ( f_h^{\mathfrak{n}} - m_{0h}^0 )\|_{L^2(\Omega)},
\eal
\ee
where the constant $c=c'\alpha$ with
\be
\alpha = 1 + \frac{\sqrt{2}}{R'_{\min}} \max_{\ell} \|R_\ell\|_{L^\infty(\Omega_\varepsilon)} \sum_{\ell=1}^M \|\Pi P_\ell\|_{L^2(\Omega_\mu)}.
\ee
By applying (\ref{ffeqbdd}) recursively, it gives the estimate (\ref{ffeqbdd0}).
\end{proof}

By Proposition \ref{fullDG2lem}, it follows that the 
the full rank DG solution $f_h^\mathfrak{n}$ converges to the zeroth moment of the projection $f_h^0 \in V_h$ of the initial solution, namely, the equilibrium solution  is given by
\be\label{eqiso}
f_h^\teq = m_{0h}^0.
\ee
From (\ref{isopartcons}), if we further truncate the initial data as $\hat f_h^0 \in V_h$, then 
the equilibrium solution in (\ref{eqiso}) will become
\be\label{eqisom}
f_h^\teq = \hat m_{0h}^0 = \frac{1}{2}\int_{\Omega_\mu} \hat f_h^0 d\mu.
\ee
We denote by $\hat f_h^\teq = X(\mu)^T\hat F^\teq Y(\varepsilon)$, then we have by Proposition \ref{prop2.2},
\be
F^\teq = \frac{1}{2} L_0L_0^T \hat F^0.
\ee

\begin{remark}
From (\ref{Lstab}) in Proposition \ref{fullDG1lem} and (\ref{ffeqbdd0}) in Proposition \ref{fullDG2lem}, we can find as $\Delta t$ is sufficiently large, the convergence rate of $f_h^{\mathfrak{n}}$ to the corresponding equilibrium solution is $O\left(\left(\frac{1}{\Delta t}\right)^\mathfrak{n}\right)$. In particular, the convergence rate of $f_h^1$ is $O\left(\frac{1}{\Delta t}\right)$.
\end{remark}

\iffalse % please don't delete this part
Note that $f_h^\teq = X(\mu)^T F^\teq Y(\varepsilon)$, then by (\ref{fhexpress}), Proposition \ref{prop2.1}, and Corollary \ref{bilform}, it is easy to verify that
\be
F^\teq = \frac{1}{2} L_0 L_0^T F^0.
\ee


We denote by $f_h^\teq=X(\mu)F^\teq Y(\varepsilon) \in V_h$ the approximation of the equilibrium solution satisfying 
\be\label{Aisoeq}
\mathcal{A}_{\Iso}(f_h^\teq,w_h) 
= 0, \quad \forall w_h \in V_h,
\ee
where $\mathcal{A}_{\Iso}(\cdot, \cdot)$ is given by (\ref{bifs2}). By setting $w_h = \Pi P_\ell(\mu) w_\varepsilon$ for any $w_\varepsilon \in V_{\varepsilon,h}$, we have
\be
\bal
& \left( \varepsilon^2 \left(R_0(\varepsilon) - \frac{1}{2l+1}R_l(\varepsilon) \right) m_{\ell h}^\teq(\varepsilon), w_\varepsilon \right)_{\Omega_\varepsilon} =  0, \quad 1\leq \ell \leq k,\\
& \left( \varepsilon^2 \left(R_0(\varepsilon) - \|\Pi P_\ell\|^2_{L^2(\mathbb{S}^1)}R_l(\varepsilon) \right) m_{\ell h}^\teq(\varepsilon), w_\varepsilon \right)_{\Omega_\varepsilon} \\
& +\sum_{\ell'=k+1, \ell'\not=\ell}^M \frac{1}{2} \left(\varepsilon^2R_{\ell'}(\varepsilon) (\Pi P_l, \Pi P_{\ell'})_{L^2(\mathbb{S}^1)}m_{\ell' h}^\teq(\varepsilon), w_\varepsilon\right)_{\Omega} =  0, \quad k+1\leq \ell \leq M.
\eal
\ee
Let $w_\varepsilon = m_{\ell h}^\teq(\varepsilon)$, 
then for $1 \leq \ell \leq k$, we have by Assumption \ref{assumRl},
\be\label{mleq0}
m_{\ell h}^\teq(\varepsilon) = 0;
\ee
for $k+1 \leq \ell \leq M$, we have by (\ref{PiPlerr}), (\ref{assumRlp}),
\be\label{RptRm}
R'_{\min} \|\varepsilon m_{\ell h}^\teq(\varepsilon)\|_{L^2(\Omega_\varepsilon)} - \tau \max_{k+1 \leq \ell \leq M} \|R_\ell\|_{L^\infty(\Omega_\varepsilon)} \sum_{\ell'=k+1, \ell'\not=\ell}^M \|\varepsilon m_{\ell' h}^\teq(\varepsilon)\|_{L^2(\Omega_\varepsilon)} \leq 0.
\ee
Summation of (\ref{RptRm}) over $k+1 \leq \ell \leq M$ gives
\be
\left(R'_{\min} - (M-k)\tau \max_{k+1 \leq \ell \leq M} \|R_\ell\|_{L^\infty(\Omega_\varepsilon)} \right) \sum_{l=k+1}^M \|\varepsilon m_{\ell h}^\teq(\varepsilon)\|_{L^2(\Omega_\varepsilon)} \leq 0.
\ee
As the meshes are refined such that $\tau \leq \frac{R'_{\min}}{(M-k) \max_{k+1\leq \ell \leq M}\|R_l\|_{L^\infty(\Omega_\varepsilon)} }$, then we have that (\ref{mleq0}) also holds for  $k+1 \leq \ell \leq M$.

Thus, (\ref{Aisoeq}) is equivalent to 
\be
\mathcal{A}_{\Iso}(f_h^\teq,w_h) =4\pi\left(\varepsilon^2R_0(\varepsilon) (m^\teq_{0 h}(\varepsilon)-f_h^\teq), w_h\right)_{\Omega} = 0.
\ee
Set $w_h=m_{\ell h}(\varepsilon)-f_h^\teq$, we have by Assumption \ref{assumRl},
\be
f_h^\teq = m^\teq_{0 h}(\varepsilon) = m^0_{0 h}(\varepsilon).
\ee
\fi

\subsection{Dynamical low-rank formulation}

[[[Put the semidiscrete formulation

\begin{equation}
    \partial_t {\hat{F} A}
    = P_{\hat{F}} G( \hat{F})
\end{equation}
]]]

Next, we want to present the dynamical low-rank approximation of the matrix equation (\ref{semidgmat}). To begin with, we first reformulate (\ref{semidgmat}) in the dynamical low-rank framework. 

\subsubsection{Differential equations for low-rank approximation}
We obtained a matrix differential equation (\ref{semidgmat}) for each equation (\ref{tp1})-(\ref{tp4}) subject to initial condition (\ref{tpinit}). To present its dynamic low-rank formulation, we first review the decompositions of rank-$r$ matrices and of their tangent matrices.

Let $\mathcal{M}_r \in \mathbb{R}^{m\times n}$ be the manifold of rank-$r$ matrices ($r \ll \min\{m,n\}$), then any rank-$r$ matrix $\hat{F} \in \mathbb{R}^{m\times n}$ has the decomposition
\be\label{FUSE}
\hat{F}(t) = U(t)S(t)E(t)^T,
\ee
where $S(t)\in \mathbb{R}^{r\times r}$ is nonsingular, $U(t)\in \mathbb{R}^{m\times r}$ and $E(t)\in \mathbb{R}^{n\times r}$ have (weighted) orthonormal columns 
\be\label{orthocond}
U^TU = E^TA_\varepsilon E = I_r,
\ee
in which $I_r$ is the identity matrix of dimension $r$ and $A_\varepsilon$ is the positive-definite symmetric block matrix given by (\ref{Avare}).
%Following (\ref{DGtoMatDef}), the the polynomials corresponding to $\hat{F}$ is given by
%$$
%\hat{f}_h = (XU) S (YE)^T.
%$$
\EE{Motivate keeping the weight ($A_{\varepsilon}$) separate in the matrix equation.  Note that this is slightly different from the ``standard''.}

The weighted tangent space of $\mathcal{M}_r$ is given by
\be\label{TFMr}
\mathcal{T}_{\hat{F}} \mathcal{M}_r = \{\delta USE^T+U\delta S E^T + US\delta E^T: \ \delta S \in \mathbb{R}^{r\times r}, U^T\delta U =0, E^TA_{\varepsilon}\delta E=0 \}.
\ee
We define by 
\be\label{projperp}
P_U = UU^T, \quad P_E = EE^T, \quad P_U^\perp = I_m-P_U, \quad P_E^\perp=A_{\varepsilon}^{-1}-P_E,
\ee
the orthogonal projections onto the spaces spanned by the columns of $U$, weighted orthogonal projections onto the spaces spanned by the columns of $E$, and their (weighted) orthogonal complements, respectively. It can be verified that all matrices in (\ref{projperp}) are symmetric. In particular, $P_E$ and $P_E^\perp$ satisfy
\be
\bal
& P_E^T A_\varepsilon P_E = P_E, \quad P_E^T A_\varepsilon P_E^\perp = 0, \quad E^T A_\varepsilon P_E= E^T, \quad   E^T A_\varepsilon P_E^\perp =  0, \quad \delta E^T  A_\varepsilon P_E^\perp =  \delta E^T,
\eal
\ee
where $\delta E$ is given in (\ref{TFMr}).
For any tangent matrix $\delta \hat{F} \in \mathcal{T}_{\hat{F}} \mathcal{M}_r$, it has the decomposition
\be\label{deltaF}
\delta \hat{F} = \delta USE^T+U\delta S E^T + US\delta E^T,
\ee
in which
\be
\bal
\delta S = &  U^T \delta \hat{F} A_\varepsilon E, \\
\delta U = & P_U^\perp \delta \hat{F} A_\varepsilon ES^{-1}, \\
\delta E = & P_E^\perp A_\varepsilon \delta \hat{F}^T U S^{-T}.
\eal
\ee

We seek low-rank approximation $\hat{F}\in \mathcal{M}_r$ such that $\partial_t \hat{F} \in \mathcal{T}_{\hat{F}} \mathcal{M}_r$ satisfies the minimization problem
\be\label{semidgam}
\partial_t \hat{F} A^{\varepsilon}= \argmin_{\delta \hat{F} \in \mathcal{T}_{\hat{F}} \mathcal{M}_r}\|\delta \hat{F}A_\varepsilon-G(\hat{F})\|_\mathcal{F}.
\ee
Set $J(ZA_\varepsilon) = \| ZA_\varepsilon-G(\hat{F})\|^2_\mathcal{F}$, then $J(\partial_t \hat{F}A_\varepsilon)$ is the minimum  of $J(ZA_\varepsilon)$, by the variational method, we have for any $\delta \hat{F} \in \mathcal{T}_{\hat{F}} \mathcal{M}_r$,
\be
\bal
\frac{d}{d\beta} J(\partial_t \hat{F}A_\varepsilon + \beta \delta \hat{F} )|_{\beta=0}= 2\left(\partial_t \hat{F} A^{\varepsilon}- G(\hat{F}), \delta \hat{F} \right )_\mathcal{F} = 0,
\eal
\ee
which implies that the minimization condition (\ref{semidgam}) on $\mathcal{T}_{\hat{F}} \mathcal{M}_r$ is equivalent to the following Galerkin equation, finding $\partial_t \hat{F} \in \mathcal{T}_{\hat{F}} \mathcal{M}_r$ such that
\be\label{Fglaerkin}
\left ( \partial_t \hat{F}A_{\varepsilon}- G(\hat{F}), \delta \hat{F}\right)_\mathcal{F}=0, \quad \forall \delta \hat{F} \in \mathcal{T}_{\hat{F}} \mathcal{M}_r.
\ee

In the following, we derive differential equations for the factors in the representation (\ref{FUSE}).
\begin{proposition}\label{diffprop}
For $\hat{F} = USE^T \in \mathcal{M}_r$ with nonsingular $S\in \bbR^{r\times r}$, the basis $U \in \bbR^{m\times r}$ and $E\in \bbR^{n\times r}$ satisfying (\ref{orthocond}), then 
under the gauge condition
\be\label{gaugecond}
U^T\dot{U} =0, \quad E^TA_{\varepsilon}\dot{E}=0,
\ee
the minimization problem (\ref{semidgam}) or the equation (\ref{Fglaerkin}) is equivalent to 
\be\label{dotF}
\partial_t \hat{F} = \dot{U}SE^T+U\dot{S}E^T+US\dot{E}^T,
\ee
where
\begin{subequations}\label{dotUSE}
\begin{align}
\dot{S} = & U^TG(\hat{F})E,\\
\dot{U} = & P_U^\perp G(\hat{F}) ES^{-1}, \\
\dot{E} = & P_E^\perp G(\hat{F})^T US^{-T}.
\end{align}
\end{subequations}
Here $P_U^\perp$ and $P_E^\perp$ are defined in (\ref{projperp}).
\end{proposition}
\begin{proof}
We first substitute $\delta \hat{F}=U\delta SE^T$, and this is of the form (\ref{deltaF}) with $\delta U =0$,  $\delta E = 0$, then we have
\be\label{Fglaerkin1}
\left ( \partial_t \hat{F}A_{\varepsilon}- G(\hat{F}), U\delta S E^T \right)_\mathcal{F}=0.
\ee
By Lemma \ref{FrobProp}, (\ref{Fglaerkin1}) is equivalent to
\be\label{Fglaerkin2}
\left ( U^T\left(\partial_t \hat{F}A_{\varepsilon}- G(\hat{F}) \right)E,\delta S\right)_\mathcal{F}=0.
\ee
Since $\delta S$ is arbitrary, we have
\be
U^T\left(\partial_t \hat{F}A_{\varepsilon}- G(\hat{F}) \right)E = 0.
\ee
By replacing $\partial_t \hat{F}$ by (\ref{dotF}) and using the conditions (\ref{orthocond}) and (\ref{gaugecond}), we obtain (\ref{dotUSE}a).
Similarly, taking $\delta Y = \delta U S E^T$ with $U^T\delta U =0$, we obtain (\ref{dotUSE}b). Finally, taking $\delta Y = US\delta E^T$ with $E^TA_\varepsilon \delta E=0$, we obtain (\ref{dotUSE}c).
\end{proof}
By Proposition \ref{diffprop}, condition (\ref{Fglaerkin}) can be written as the differential equation on the weighted tangent space $\mathcal{T}_{\hat{F}} \mathcal{M}_r$,
\be\label{lrode}
\partial_t \hat{F}A_{\varepsilon} = P(\hat{F}) G(\hat{F}),
\ee
where $P(\hat{F})$ is the weighted orthogonal projection onto the weighted tangent space $\mathcal{T}_{\hat{F}} \mathcal{M}_r$, and it can be written as an alternating sum of three subprojections onto the weighted co-range, the intersection of weighted co-range and range, and the range of the rank-$r$ matrix $\hat{F}$, namely,
\be
\bal
P(\hat{F}) G = GEE^TA_\varepsilon - UU^TGEE^TA_\varepsilon + UU^TG, \quad G\in \mathbb{R}^{m \times n}.
\eal
\ee
%Moreover, if $Z\in \mathcal{T}_{\hat{F}} \mathcal{M}_r$, it can be verified that
%$$
%P(\hat{F}) Z= Z.
%$$

To obtain the initial data for (\ref{lrode}), we first 
apply singular value decomposition (SVD) to $F(0)$ and truncate
$$
{F}(0) =  U^0 \tilde S^0  (\tilde E^0)^T, 
$$
where $ U^0 \in \mathbb{R}^{m\times r}$, $\tilde S^0 \in \mathbb{R}^{r\times r}$, and $\tilde E^0 \in \mathbb{R}^{n\times r}$ satisfying $(U^0)^TU^0=I_{r}$ and $(\tilde E^0)^T\tilde E^0=I_{r}$.
Next, we apply the weighted Gram-Schmidt decomposition (Algorithm \ref{qrw} or Algorithm \ref{qrm}) to $\tilde{E}^0$ and obtain
\be
\tilde{E}^0 = E^0 R^0,
\ee
where $R^0 \in \mathbb{R}^{r \times r}$, $E^0 \in \mathbb{R}^{n \times r}$ satisfies 
\be\label{E0cond}
(E^0)^T A_\varepsilon E^0 = I_{r}.
\ee
The initial condition associated with (\ref{lrode}) is taken as
\be\label{initdecomp}
\hat{F}(0) = U^0S^0(E^0)^T,
\ee
where $S^0= \tilde{S}^0 (R^0)^T \in \mathbb{R}^{r\times r}$.

By taking $\mathbf{K}=US$, $\mathbf{L}=ES^T$, then the semi-discrete dynamical low-rank matrix equation (\ref{lrode}) can be equivalently written as
\begin{subequations}\label{semiDLRMat}
\begin{align}
\partial_t (\mathbf{K}) = & G(\mathbf{K}E^T) E, \\
\partial_t (\mathbf{L}) = & A_\varepsilon^{-1} G(U\mathbf{L}^T)^T U,\\
\partial_t {S} = & U^TG(USE^T)E,
\end{align}
\end{subequations}
subject to the initial data
\be
\mathbf{K}(0) = U^0S^0, \quad \mathbf{L}(0) = E^0(S^0)^T, \quad S(0) = S^0. 
\ee

\subsubsection{Semi-discrete dynamical low-rank DG scheme}
Now we give the equivalent formulation of the dynamical low-rank formulation (\ref{lrode}) or (\ref{semiDLRMat}) in DG framework. To begin with, we define three subspaces of the DG finite element space $V_h$,
\begin{subequations}\label{subspaces0}
\begin{align}
V_{\bK}=& \left\{v \ | \ v=  X(\mu)^T\mathbf{K}(E)^T Y(\varepsilon), \quad E^TA_\varepsilon\dot{E}=0, \ \forall \mathbf{K} \in \mathbb{R}^{m\times r} \right\}, \\
V_{\mathbf{L}}= & \left\{v \ | \ v=  X(\mu)^TU\mathbf{L}^T Y(\varepsilon), \quad U\dot{U}=0, \ \forall \mathbf{L} \in \mathbb{R}^{n\times r} \right\},\\
V_{S}=& \left\{v \ | \ v=X(\mu)^TUSE^T Y(\varepsilon), \quad \quad U\dot{U}=0, \ E^TA_\varepsilon\dot{E}=0, \ \forall S \in \mathbb{R}^{r\times r} \right\},
\end{align}
\end{subequations}

The semi-discrete dynamical low-rank DG formulation is to find \be\label{lrdgsol0}
\bal
f_\mathbf{K}= & X(\mu)^T{\mathbf{K}}^{*}E^T Y(\varepsilon) \in V_{\bK},\\
f_\mathbf{L} = & X(\mu)^TU({\mathbf{L}}^{*})^T Y(\varepsilon) \in V_{\mathbf{L}},\\
f_S= & X(\mu)^TU{S}^{*}E^T Y(\varepsilon) \in V_{S},
\eal
\ee
such that
\begin{subequations}\label{semiDLRDG}
\begin{align}
\left(\partial_t f_\mathbf{K}, w_1;\varepsilon^2 \right)_{\Omega} = & \mathcal{A}(f_\mathbf{K}, w_1), \quad \forall w_1 \in V_{\bK},\\
\left(\partial_t f_\mathbf{L}, w_2;\varepsilon^2 \right)_{\Omega} = & \mathcal{A}(f_\mathbf{L}, w_2), \quad \forall w_2 \in V_{\mathbf{L}},\\
\left(\partial_t f_S, w_3;\varepsilon^2 \right)_{\Omega} = & \mathcal{A}(f_S, w_3), \quad \forall w_3 \in V_{S},
\end{align}
\end{subequations}
where $\mathcal{A}(\cdot, \cdot)$ is given by (\ref{bifs1}) for equation (\ref{tp1}) and by (\ref{bifs2}) for equation (\ref{tp2}), respectively.
(\ref{semiDLRDG}) is subject to the initial condition
\be
f_\mathbf{K}(0) = f_\mathbf{L}(0) = f_S^\mathfrak{n}(0) = \hat{f}_h(0)= X(\mu)^T\hat F(0)Y(\varepsilon).
\ee

Here the solutions of the semi-discrete DG scheme s (\ref{semiDLRDG}) for equation (\ref{tp1}) and (\ref{tp2}) share the same stability as the semi-discrete DG scheme (\ref{semiDG}).

\begin{lemma}
Let $({\mathbf{K}}^{*}, {\mathbf{L}}^{*}, {S}^{*})$ be the coefficient matrix set of the solution set $(f_\mathbf{K}, f_\mathbf{L}, f_S)$ of the semi-discrete dynamical low-rank DG scheme (\ref{semiDLRDG}), then it follows
\be
 {\mathbf{K}}^{*}={\mathbf{K}}, \quad {\mathbf{L}}^{*}={\mathbf{L}}, \quad {S}^{*}=S,
\ee
where $({\mathbf{K}}, {\mathbf{L}}, {S})$ is the solution set of the system (\ref{semiDLRMat}).
\end{lemma}
\begin{proof}
By Corollary \ref{bilform}, the matrix equation for (\ref{semiDLRDG}) is equivalent to finding $\mathbf{K}^{*} \in \mathbb{R}^{m\times r}$, $\mathbf{L}^{*} \in \mathbb{R}^{n\times r}$, and $S^{*} \in \mathbb{R}^{r\times r}$ such that for any $\mathbf{K}_W\in \mathbb{R}^{m\times r}$, $\mathbf{L}_W\in \mathbb{R}^{n\times r}$, and $S_W\in \mathbb{R}^{m\times r}$,
\be\label{semimatodeK}
\bal
\left(\partial_t(\mathbf{K}^* E^T) A_{\varepsilon}, \mathbf{K}_WE^T \right)_\mathcal{F}
= & \left(G(\mathbf{K}^{*}E^T), \mathbf{K}_WE^T\right)_\mathcal{F},\\
\left( \partial_t (U (\mathbf{L}^*)^T) A_{\varepsilon}, U\mathbf{L}_W^T \right)_\mathcal{F}
= & \left(G(U(\mathbf{L}^{*})^T), U\mathbf{L}_W^T\right)_\mathcal{F},\\
\left( \partial_t( US^*E^T) A_{\varepsilon}, US_WE^T \right)_\mathcal{F}
= & \left( G(US^*E^T), US_WE^T\right)_\mathcal{F}.
\eal
\ee
By the condition (\ref{gaugecond}) and Lemma \ref{FrobProp}, the matrix equation (\ref{semimatodeK}) is equivalent to 
\be\label{semimatodeK0}
\bal
\left(\partial_t \mathbf{K}^*, \mathbf{K}_W \right)_\mathcal{F}
= & \left(G(\mathbf{K}^{*}E^T)E, \mathbf{K}_W\right)_\mathcal{F},\\
\left( \partial_t (\mathbf{L}^*)^T A_{\varepsilon}, \mathbf{L}_W^T \right)_\mathcal{F}
= & \left(U^TG(U(\mathbf{L}^{*})^T), \mathbf{L}_W^T\right)_\mathcal{F},\\
\left( \partial_tS^*, S_W \right)_\mathcal{F}
= & \left( U^TG(US^*E^T)E, S_W\right)_\mathcal{F}.
\eal
\ee
By the arbitrariness of $\mathbf{K}_W, \mathbf{L}_W$, and $S_W$, we have
\be\label{semimatodeK1}
\bal
\partial_t \mathbf{K}^*
= & G(\mathbf{K}^{*}E^T)E,\\
\partial_t \mathbf{L}^* 
= & A_{\varepsilon}^{-1}G(U(\mathbf{L}^{*})^T)^TU,\\
\partial_tS^*
= & U^TG(US^*E^T)E.
\eal
\ee
Since the ODE systems (\ref{semiDLRMat}) and (\ref{semimatodeK1}) share the same initial data, so the conclusion holds.
\end{proof}


\subsection{Unconventional integrator}

[[[Write down the explicit UI.]]]
Following [UI] paper, we can easily present an explicit unconventional integrator to solve the differential equation (\ref{lrode}). The one time integration from 
$t_{\mathfrak{n}}$ to $t_{\mathfrak{n}+1} = t_\mathfrak{n}+\Delta t$ can be summarized as follows. 
\begin{alg}\label{lralgex}
An unconventional integrator with explicit forward Euler time discretization.
\begin{itemize}
    \item{\textbf{Step 1:}} Update $U^\mathfrak{n} \rightarrow U^{\mathfrak{n}+1}$ and $E^\mathfrak{n} \rightarrow E^{\mathfrak{n}+1}$ in parallel:
\begin{itemize}
    \item{\textbf{K-step}:} Solve the $m\times r$ matrix equation
    \be\label{kstepex}
    \frac{\mathbf{K}^{\mathfrak{n}+1}-\mathbf{K}^\mathfrak{n}}{\Delta t} = G(\mathbf{K}^{\mathfrak{n}}(E^\mathfrak{n})^T)E^\mathfrak{n}, \quad \mathbf{K}^\mathfrak{n}=U^\mathfrak{n}S^\mathfrak{n}.
    \ee
    Perform a QR factorization $\mathbf{K}^{\mathfrak{n}+1}=U^{\mathfrak{n}+1}R^{\mathfrak{n}+1}$ and compute the $r \times r$ matrix $M^{\mathfrak{n}+1}=(U^{\mathfrak{n}+1})^T U^\mathfrak{n}$.
    \item{\textbf{L-step}:} Solve the $n\times r$ matrix equation
    \be\label{lstepex}
    \frac{\mathbf{L}^{\mathfrak{n}+1}-\mathbf{L}^\mathfrak{n}}{\Delta t} = {A}_\varepsilon^{-1}G(U^\mathfrak{n}(\mathbf{L}^{\mathfrak{n}})^T)^TU^\mathfrak{n}, \quad \mathbf{L}^\mathfrak{n}=E^\mathfrak{n}(S^\mathfrak{n})^T.
    \ee
    Perform a QR factorization $\mathbf{L}^{\mathfrak{n}+1}=\tilde E^{\mathfrak{n}+1}\tilde R^{\mathfrak{n}+1}$, then decompose $\tilde E^{\mathfrak{n}+1}$ by Algorithm \ref{qrm} to obtain $\tilde E^{\mathfrak{n}+1} = E^{\mathfrak{n}+1} \tilde{\tilde{R}}^{\mathfrak{n}+1}$, and compute the $r \times r$ matrix $N^{\mathfrak{n}+1}=(E^{\mathfrak{n}+1})^T A_\varepsilon E^\mathfrak{n}$.
\end{itemize}
   \item{\textbf{Step 2:}} Update $S^\mathfrak{n}\rightarrow S^{\mathfrak{n}+1}$:
   \begin{itemize}
       \item{\textbf{S-step}:} Solve the $r\times r$ matrix equation
    \be\label{sstepex}
    \frac{{S}^{\mathfrak{n}+1}-\mathbf{S}^\mathfrak{n}}{\Delta t} = (U^{\mathfrak{n}+1})^T(G(U^{\mathfrak{n}+1}S^{\mathfrak{n}} (E^{\mathfrak{n}+1})^T)E^{\mathfrak{n}+1}, \quad \mathbf{S}^\mathfrak{n}=M^{\mathfrak{n}+1}S^\mathfrak{n}(N^{\mathfrak{n}+1})^T.
    \ee
   \end{itemize}
\end{itemize}
\end{alg}
In Algorithm \ref{lralgex},  $G=G_1$ for problem (\ref{tp1}) and $G=G_2$ for problem (\ref{tp2}).
The existence and uniqueness of the solution for each equation in  Algorithm \ref{lralgex} is obvious. However, the time step need to satisfy certain CFL condition, and an explicit scheme for equation (\ref{tp2}) does not preserve the total number of the particles.

==> archive/LinearConservative.tex <==
\section{Conservative formulation for scattering}

%[[[]Why is this important?  What other work has been done?]]]

%\subsection{The DLR solution for problem (\ref{tp2})}
%For Eq. (\ref{tp2}), Theorem \ref{KLSexist} shows that Algorithm \ref{lralg} admits a unique solution set, or equivalently, the first order DG scheme (\ref{fullDG1K}) admits a unique dynamical low-rank DG solution $\hat{f}_h^{\mathfrak{n}} \in V_{S^{\mathfrak{n}}}$, for which we also have the following stability result.

The solution of Eq. (\ref{tp2}) converges to its zeroth moment and conserves the total number of particles. The equations in Algorithm \ref{lralg} for Eq. (\ref{tp2}) are well-posed, but the associated dynamical low-rank DG solution may not conserve the zeroth moment and the total number of particles, which may result in the solution converging to a wrong equilibrium solution. 

\subsection{A truncation conservative algorithm}

%[[[]Put in our method and Einkemmer's.  Discuss differences.]]]

A conservative dynamical low-rank algorithm was proposed in \cite{einkemmer2022} for the Vlasov--Poisson equation, the strategy in a one-time step includes adding a set of basis functions to the approximation space and a conservative truncation. 
Based on this strategy, we can modify Algorithm \ref{lralg} as follows.

\begin{alg}\label{lralgctp2E}
A conservative semi-implicit unconventional integrator for equation (\ref{tp2}) following the conservative strategy in \cite{einkemmer2022}:
\begin{itemize}
\item{\textbf{Step 1:}} The same initialization as Algorithm \ref{lralgtp1} Step 1, and set $U^{0} = [U^\teq, U^{0}_{rem}]$.
    \item{\textbf{Step 2:}} Update $U^\mathfrak{n} \rightarrow \tilde U^{\mathfrak{n}+1}$ and $E^\mathfrak{n} \rightarrow \tilde E^{\mathfrak{n}+1}$ in parallel:
\begin{itemize}
    \item{\textbf{K-step}:} Solve the $m\times r' $ matrix equation (\ref{kstep});\\
    Set $\tilde{\mathbf{K}}^{\mathfrak{n}+1} = [U^\teq, \mathbf{K}^{\mathfrak{n}+1}, U^0_{rem}]$; \\
    Perform a QR decomposition $\tilde{\mathbf{K}}^{\mathfrak{n}+1} = \tilde U^{\mathfrak{n}+1} R^{\mathfrak{n}+1}$, compute the $2r'\times r'$ matrix $M^{\mathfrak{n}+1}=(\tilde U^{\mathfrak{n}+1})^T U^\mathfrak{n}$, and set $\tilde U^{\mathfrak{n}+1} = [U^\teq, \tilde U^{\mathfrak{n}+1}_{rem}]$.
    \item{\textbf{L-step}:} Solve the $n\times r'$ matrix equation (\ref{lstep});\\
    Set $\tilde{\mathbf{L}}^{\mathfrak{n}+1} = [\mathbf{L}^{\mathfrak{n}+1}, E^\mathfrak{n}]$; \\
    Perform decomposition in Algorithm \ref{qrw} such that  $\tilde{\mathbf{L}}^{\mathfrak{n}+1}= \tilde{E}^{\mathfrak{n}+1} \tilde{R}^{\mathfrak{n}+1}$, and compute the $2r' \times r'$ matrix $N^{\mathfrak{n}+1}=(\tilde E^{\mathfrak{n}+1})^T A_\varepsilon E^\mathfrak{n}$.
\end{itemize}
   \item{\textbf{Step 3:}} Update $S^\mathfrak{n}\rightarrow \tilde S^{\mathfrak{n}+1}$:
   \begin{itemize}
       \item{\textbf{S-step}:} Solve the $2r'\times 2r'$ matrix equation (\ref{sstep})  with $U^{\mathfrak{n}+1}$, $E^{\mathfrak{n}+1}$, and  $S^{\mathfrak{n}+1}$ replaced by $\tilde U^{\mathfrak{n}+1}$, $\tilde U^{\mathfrak{n}+1}$, and $\tilde S^{\mathfrak{n}+1}$, respectively.
   \end{itemize}
   \item{\textbf{Step 4:}} Conservative truncation to rank $r'$. %$\tilde{E}^{\mathfrak{n}+1} \rightarrow {E}^{\mathfrak{n}+1}$.
   \begin{itemize}
        \item Compute $\bar{\mathbf{L}}^{\mathfrak{n}+1} =  \tilde{E}^{\mathfrak{n}+1} (\tilde{S}^{\mathfrak{n}+1})^T$ and distribute it into two parts,
        \be\label{LLL}
        \bar{\mathbf{L}}^{\mathfrak{n}+1} = [\bar{\mathbf{L}}^{\mathfrak{n}+1}_{cons}, \bar{\mathbf{L}}^{\mathfrak{n}+1}_{rem}],
        \ee
        where $\bar{\mathbf{L}}^{\mathfrak{n}+1}_{cons} \in \mathbb{R}^{n\times 1}$, $\bar{\mathbf{L}}^{\mathfrak{n}+1}_{rem} \in \mathbb{R}^{n\times (2r'-1)}$.
        \item Apply the decomposition Algorithm \ref{qrw} to $\bar{\mathbf{L}}^{\mathfrak{n}+1}_1$ and obtain
        \be\label{Lconsdecom}
        \bar{\mathbf{L}}^{\mathfrak{n}+1}_{cons} = E^{\mathfrak{n}+1}_{cons} S^{\mathfrak{n}+1}_{cons}.
        \ee
        \item Apply the decomposition Algorithm \ref{qrw} to $\bar{\mathbf{L}}^{\mathfrak{n}+1}_{rem}$, and obtain
        \be
        \bar{\mathbf{L}}^{\mathfrak{n}+1}_{rem} = \bar E^{\mathfrak{n}+1}_{rem} \bar S^{\mathfrak{n}+1}_{rem}.
        \ee
        \item  Apply the SVD decomposition to $(\bar S^{\mathfrak{n}+1}_{rem})^T$ and truncate $S^{\mathfrak{n}+1}_{rem} \in \mathbb{R}^{(r'-1)\times (r'-1)}$,
       \be\label{trunerr}
        (\bar S^{\mathfrak{n}+1}_{rem})^T \approx U^* S^{\mathfrak{n}+1}_{rem} (E^*)^T,
       \ee
       and compute 
       \be
       U^{\mathfrak{n}+1}_{rem} = \tilde U^{\mathfrak{n}+1}_{rem} U^*, \quad E^{\mathfrak{n}+1}_{rem} = \bar E^{\mathfrak{n}+1}_{rem} E^*.
       \ee
       \item Set $U^{\mathfrak{n}+1} = [U^\teq, U^{\mathfrak{n}+1}_{rem}]$.
      \item Set $\bar E^{\mathfrak{n}+1} = [E^{\mathfrak{n}+1}_{cons}, E^{\mathfrak{n}+1}_{rem}]$ and apply Algorithm \ref{qrw} for 
      \be\label{EbarE}
      \bar E^{\mathfrak{n}+1}=E^{\mathfrak{n}+1} R^{\mathfrak{n}+1}.
      \ee
      \item Set 
      \begin{equation}\label{Sn1decom}
S^{\mathfrak{n}+1} = 
\begin{bmatrix}
S^{\mathfrak{n}+1}_{cons} & 0 \\
0 & S^{\mathfrak{n}+1}_{rem} \\
\end{bmatrix}
(R^{\mathfrak{n}+1})^T.
\end{equation}
   \end{itemize}
\end{itemize}
\end{alg}

It can be proved that Algorithm \ref{lralgctp2E} conserves the zeroth moment, and so do the total number of particles.

\subsection{A modified truncation conservative algorithm with less unknowns}
Based on the observation, we can further reduce the total number of unknowns in Algorithm \ref{lralgctp2E} and still conserve the zeroth moment and the total number of particles. 

In the following, we first go through how are the equations in Algorithm \ref{lralg} being solved.
For convenience, we denote by
\be
\widetilde{A}_\ell^{\Iso,\mathfrak{n}} = (E^\mathfrak{n})^T A^{\Iso}_{\ell} E^\mathfrak{n}.
\ee

For (\ref{kstep}), we have 
\be\label{tp2kstep}
\frac{\mathbf{K}^{\mathfrak{n}+1}-\mathbf{K}^\mathfrak{n}}{\Delta t} = G_2(\mathbf{K}^{\mathfrak{n}+1}(E^\mathfrak{n})^T)E^\mathfrak{n} = 2\pi \sum_{\ell=0}^M L_{\ell} L_{\ell}^T \mathbf{K}^{\mathfrak{n}+1}\widetilde{A}_\ell^{\Iso,\mathfrak{n}} -4\pi \mathbf{K}_\ell^{\mathfrak{n}+1}\widetilde{A}_0^{\Iso,\mathfrak{n}}.
\ee
We denote by $\widetilde{\mathbf{K}}_\ell^{\mathfrak{n}}=L_{\ell}^T\mathbf{K}^{\mathfrak{n}}$, then 
left-multiplying (\ref{tp2kstep}) by the vectors $L_{\ell'}^T$, $\ell'=0, \cdots, M$, and applying (\ref{Lmulprop}), it follows
\be\label{tp2kstep1}
\frac{\widetilde{\mathbf{K}}^{\mathfrak{n}+1}_\ell-\widetilde{\mathbf{K}}^\mathfrak{n}_\ell}{\Delta t} =\frac{4\pi}{2\ell+1}  \widetilde{\mathbf{K}}^{\mathfrak{n}+1}_\ell \widetilde{A}_\ell^{\Iso,\mathfrak{n}} -4\pi \widetilde{\mathbf{K}}_\ell^{\mathfrak{n}+1}\widetilde{A}_0^{\Iso,\mathfrak{n}}.
\ee
From (\ref{tp2kstep1}), we obtain for $\ell=0,\cdots, M$,
\be\label{tp2kstep2}
\widetilde{\mathbf{K}}^{\mathfrak{n}+1}_\ell= \widetilde{\mathbf{K}}^{\mathfrak{n}}_\ell \left(I_{r} + 4\pi\Delta t \left( \widetilde{A}_0^{\Iso,\mathfrak{n}} - \frac{1}{2\ell+1} \widetilde{A}_\ell^{\Iso,\mathfrak{n}} \right) \right)^{-1}.
\ee
Thus, we can obtain $\bK^{\mathfrak{n}+1}$ from (\ref{tp2kstep}) by treating $\widetilde{\mathbf{K}}^{\mathfrak{n}+1}_\ell$ as known vectors, 
\be\label{tp2kstep3}
\mathbf{K}^{\mathfrak{n}+1}  = \left( \mathbf{K}^{\mathfrak{n}} + 2\pi\Delta t \sum_{\ell=0}^M L_{\ell} \left(\widetilde{\mathbf{K}}^{\mathfrak{n}+1}_\ell \widetilde{A}_\ell^{\Iso,\mathfrak{n}}\right) \right)\left(I_{r}+ 4\pi \Delta t \widetilde{A}_0^{\Iso,\mathfrak{n}} \right)^{-1}.
\ee

For (\ref{lstep}), we have 
\be\label{tp2lstep}
\frac{\mathbf{L}^{\mathfrak{n}+1}-\mathbf{L}^\mathfrak{n}}{\Delta t} = A_\varepsilon^{-1} G_2(U^\mathfrak{n}(\mathbf{L}^{\mathfrak{n}+1})^T)^TU^\mathfrak{n}= 2\pi \sum_{\ell=0}^M A_{\varepsilon}^{-1}A^{\Iso}_{\ell} \mathbf{L}^{\mathfrak{n}+1}(L_{\ell}^TU^\mathfrak{n})^T L_{\ell}^T U^\mathfrak{n} -4\pi A_{\varepsilon}^{-1}A^{\Iso}_{0} \mathbf{L}^{\mathfrak{n}+1}.
\ee
We denote by $\widetilde{\mathbf{L}}_\ell^{\mathfrak{n}+1} = \mathbf{L}^{\mathfrak{n}+1}(L_{\ell}^TU^\mathfrak{n})^T$ and $\widetilde{\mathbf{L}}_\ell^{\mathfrak{n}} = \mathbf{L}^{\mathfrak{n}}(L_{\ell}^TU^\mathfrak{n})^T$, then right-multiplying (\ref{tp2lstep}) by the column vectors $(L_{\ell'}^TU^\mathfrak{n})^T \in \mathbb{R}^{r \times 1}$, $\ell'=0, \cdots, M$, it follows
%To solve (\ref{tp2lstep}), we first consider the following equation,
\be\label{tp2lstep1}
\frac{\widetilde{\mathbf{L}}_{\ell'}^{\mathfrak{n}+1}-\widetilde{\mathbf{L}}_{\ell'}^{\mathfrak{n}}}{\Delta t} = 2\pi \sum_{l=0}^M \alpha_{\ell'\ell}^\mathfrak{n} A_{\varepsilon}^{-1}A^{\Iso}_{\ell} \widetilde{\mathbf{L}}_{\ell}^{\mathfrak{n}+1} -4\pi A_{\varepsilon}^{-1}A^{\Iso}_{0} \widetilde{\mathbf{L}}_{\ell'}^{\mathfrak{n}+1},
\ee
where the the scalar
$$
\alpha_{\ell'\ell}^\mathfrak{n} = L_{\ell}^T U^\mathfrak{n} (L_{\ell'}^TU^\mathfrak{n})^T.
$$
Therefore, we can first pre-evaluate $\widetilde{\mathbf{L}}_{\ell}^{\mathfrak{n}+1}$ by solving the linear system (\ref{tp2lstep1}).
%\be\label{tp2lstep2}
%\mathbf{L}^{1}(U^0)^TL_{\ell} = \left( I_{n\times n} + 4\pi \Delta t \left( A_{\varepsilon}^{-1}A^{\Iso}_{\varepsilon,0} - \frac{1}{2l+1} A_{\varepsilon}^{-1}A^{\Iso}_{\varepsilon,l} \right) \right)^{-1} \mathbf{L}^{0}\left((U^0)^TL_{\ell}\right).
%\ee
From (\ref{tp2lstep}), we obtain
\be\label{tp2lstep3}
\mathbf{L}^{\mathfrak{n}+1} =  \left(I_{n} +4\pi\Delta t  A_{\varepsilon}^{-1}A^{\Iso}_{0} \right)^{-1} \left( \mathbf{L}^{\mathfrak{n}} + 2\pi \Delta t \sum_{\ell=0}^M A_{\varepsilon}^{-1}A^{\Iso}_{\ell} \widetilde{\mathbf{L}}_{\ell}^{\mathfrak{n}+1} (L_{\ell}^T U^\mathfrak{n}) \right).
\ee

For (\ref{sstep}), we have 
\be\label{tp2sstep}
\bal
\frac{{S}^{\mathfrak{n}+1}-\mathbf{S}^\mathfrak{n}}{\Delta t} = &  (U^{\mathfrak{n}+1})^T(G_2(U^{\mathfrak{n}+1}S^{\mathfrak{n}+1} (E^{\mathfrak{n}+1})^T)E^{\mathfrak{n}+1}\\
%\frac{{S}^{1}-{S}^0}{\Delta t} = & (U^{1})^T G(U^{1}{S}^{1} (E^{1})^T )E^{1} \\
= & 2\pi \sum_{\ell=0}^M ( L_{\ell}^T U^{\mathfrak{n}+1})^T  L_{\ell}^T U^{\mathfrak{n}+1}{S}^{\mathfrak{n}+1} \widetilde{A}_\ell^{\Iso,\mathfrak{n}+1} -4\pi {S}^{\mathfrak{n}+1} \widetilde{A}_0^{\Iso,\mathfrak{n}+1}.
\eal
\ee
We denote by 
\be\label{Smoment}
\widetilde{S}_\ell^{\mathfrak{n}+1}=L_{\ell}^T U^{\mathfrak{n}+1}{S}^{\mathfrak{n}+1}, \quad \widetilde{\mathbf{S}}_\ell^{n}=L_{\ell}^T U^{\mathfrak{n}+1}{\mathbf{S}}^{\mathfrak{n}}, 
\ee
then left-multiplying (\ref{tp2sstep}) by the row vectors $L_{\ell'}^T U^{\mathfrak{n}+1}$, $l'=0,\cdots,M$, it follows
\be\label{tp2sstep1}
\bal
\frac{\widetilde{S}_{\ell'}^{\mathfrak{n}+1}-\widetilde{\mathbf{S}}_{\ell'}^{\mathfrak{n}}}{\Delta t} = & 2\pi \sum_{\ell=0}^M \alpha_{\ell \ell'}^{\mathfrak{n}+1} \widetilde{S}_\ell^{\mathfrak{n}+1} \widetilde{A}_\ell^{\Iso,\mathfrak{n}+1}
-4\pi \widetilde{S}_{\ell'}^{\mathfrak{n}+1} \widetilde{A}_0^{\Iso,\mathfrak{n}+1}.
\eal
\ee
So that we can also pre-evaluate $\widetilde{S}_\ell^{\mathfrak{n}+1}$ by solving the linear system (\ref{tp2sstep1}).
%By (\ref{tp2sstep1}) and Lemma \ref{Lmulprop}, we can first pre-evaluate
%\be\label{tp2sstep2}
%\bal
%L_{\ell}^TU^{1}{S}^{1} = \left((L_{\ell}^TU^{1}){S}^{0} \right) \left(I_{r\times r} + 4\pi\Delta t \left( (E^1)^T (A^{\Iso}_{\varepsilon,0}A_{\varepsilon}^{-1}) E^1 - \frac{1}{2l+1} (E^1)^T (A^{\Iso}_{\varepsilon,l}A_{\varepsilon}^{-1}) E^1 \right) \right)^{-1}.
%\eal
%\ee
From (\ref{tp2sstep}), we have
\be\label{tp2sstep3}
\bal
{S}^{\mathfrak{n}+1} =  \left( \mathbf{S}^{\mathfrak{n}} +  2\pi \Delta t \sum_{l=0}^M ( L_{\ell}^T U^{\mathfrak{n}+1})^T \widetilde{S}_\ell^{\mathfrak{n}+1} \widetilde{A}_\ell^{\Iso,\mathfrak{n}+1} \right) \left(I_{r}+4\pi\Delta t  \widetilde{A}_0^{\Iso,\mathfrak{n}+1} \right)^{-1}.
\eal
\ee

%The main property of solution to equation (\ref{tp2}) is the particle conservation (\ref{ptc}). However, the dynamical low rank solution obtained from Algorithm \ref{lralg} may not preserve it, and a remedy may be needed.
\iffalse
To proceed, we first study the basis related to the equilibrium solution $f_h^{\teq}$ of the DG scheme (\ref{fullDG1}) for equation (\ref{tp2}) satisfying
\be
\mathcal{A}_{\Iso}(f_h^{\teq},w_h)=0,
\ee
where $\mathcal{A}_{\Iso}(\cdot, \cdot)$ is given in (\ref{bifs2+}).
\fi

%In the following, we will present an alternative conservative algorithm with less unknowns and/or no truncation error. 
For ${S}^{\mathfrak{n}+1}$ and $\mathbf{S}^{\mathfrak{n}}$, we have the following result.
\begin{lemma}\label{Ubasis}
Let $U^{\mathfrak{n}+1}$ be the base in S-step for Eq. (\ref{tp2}) and $U^\teq$ be the unit vector given by (\ref{USEeq}a). If $\|(U^{\eq})^T U^{\mathfrak{n}+1}\|=1$, then it follows
\be\label{Smom}
L_0^T U^{\mathfrak{n}+1}{S}^{\mathfrak{n}+1}=L_0^T U^{\mathfrak{n}+1}{\mathbf{S}}^{\mathfrak{n}}.
\ee
\end{lemma}
\begin{proof}
By (\ref{tp2sstep1}), we have
\be\label{Smom0}
\widetilde{S}_{0}^{\mathfrak{n}+1}-\widetilde{\mathbf{S}}_{0}^{\mathfrak{n}} = 2\pi \Delta t \sum_{l=0}^M \alpha_{l0}^{\mathfrak{n}+1} \widetilde{S}_\ell^{\mathfrak{n}+1} \widetilde{A}_\ell^{\Iso,\mathfrak{n}+1}
-4\pi \Delta t\widetilde{S}_{0}^{\mathfrak{n}+1} \widetilde{A}_0^{\Iso,\mathfrak{n}+1}.
\ee
Since
\be\label{alpha0l}
\bal
\alpha_{l0}^{\mathfrak{n}+1} = & L_{0}^T U^{\mathfrak{n}+1} (L_{\ell}^TU^{\mathfrak{n}+1})^T = \|L_{0}\| (U^\teq)^T  U^{\mathfrak{n}+1} (U^{\mathfrak{n}+1})^T L_{\ell} 
=  \|L_{0}\| (U^\teq)^TL_{\ell}
= L_{0}^T L_{\ell} = 2 \delta_{0l},
\eal
\ee
where we have used Lemma \ref{uequn} for the third equality, (\ref{USEeq}) for the fourth inequality, and Lemma \ref{basisproperty} for the last equality.

By (\ref{alpha0l}), the equality (\ref{Smom0}) leads to
\be
\widetilde{S}_{0}^{\mathfrak{n}+1}-\widetilde{\mathbf{S}}_{0}^{\mathfrak{n}} = 0,
\ee
which is equivalent to (\ref{Smom}).
\end{proof}

By Lemma \ref{Ubasis} and Lemma \ref{Ebasis}, we can reduce the unknowns in Algorithm \ref{lralgctp2E}.

\begin{alg}\label{lralgctp21}
A modified conservative semi-implicit unconventional integrator for Eq. (\ref{tp2}) with less unknowns:
\begin{itemize}
\item{\textbf{Step 1:}} The same initialization as Algorithm \ref{lralgtp1} Step 1.
    \item{\textbf{Step 2:}} Update $U^\mathfrak{n} \rightarrow \tilde U^{\mathfrak{n}+1}$ and $E^\mathfrak{n} \rightarrow \tilde E^{\mathfrak{n}+1}$ in parallel:
\begin{itemize}
    \item{\textbf{K-step}:} Solve the $m\times r' $ matrix equation (\ref{kstep});\\
    Set $\tilde{\mathbf{K}}^{\mathfrak{n}+1} = [U^\teq, \mathbf{K}^{\mathfrak{n}+1}]$; \\
    Perform a QR decomposition $\tilde{\mathbf{K}}^{\mathfrak{n}+1} = \tilde U^{\mathfrak{n}+1} R^{\mathfrak{n}+1}$, compute the $(r'+1)\times r'$ matrix $M^{\mathfrak{n}+1}=(\tilde U^{\mathfrak{n}+1})^T U^\mathfrak{n}$, and set $\tilde U^{\mathfrak{n}+1} = [U^\teq, \tilde U^{\mathfrak{n}+1}_{rem}]$.
    \item{\textbf{L-step}:} Solve the $n\times r'$ matrix equation (\ref{lstep});\\
    Set $\tilde{\mathbf{L}}^{\mathfrak{n}+1} = [\mathbf{L}^{\mathfrak{n}+1}, E^\mathfrak{n}]$; \\
    Perform decomposition in Algorithm \ref{qrw} such that  $\tilde{\mathbf{L}}^{\mathfrak{n}+1}= \tilde{E}^{\mathfrak{n}+1} \tilde{R}^{\mathfrak{n}+1}$, and compute the $2r' \times r'$ matrix $N^{\mathfrak{n}+1}=(\tilde E^{\mathfrak{n}+1})^T A_\varepsilon E^\mathfrak{n}$.
\end{itemize}
   \item{\textbf{Step 3:}} Update $S^\mathfrak{n}\rightarrow \tilde S^{\mathfrak{n}+1}$:
   \begin{itemize}
       \item{\textbf{S-step}:} Solve the $(r'+1)\times 2r'$ matrix equation (\ref{sstep})  with $S^{\mathfrak{n}+1}$ replaced by $\tilde S^{\mathfrak{n}+1}$.
   \end{itemize}
   \item{\textbf{Step 4:}} Conservative truncation to rank $r'$. It is similar to the Step 4 in Algorithm \ref{lralgctp2E}, with the difference on the dimension $\bar{\mathbf{L}}^{\mathfrak{n}+1}_{rem} \in \mathbb{R}^{n\times r'}$.
\iffalse
\begin{itemize}
        \item Compute $\bar{\mathbf{L}}^{\mathfrak{n}+1} =  \tilde{E}^{\mathfrak{n}+1} (\tilde{S}^{\mathfrak{n}+1})^T$ and distribute it into two parts,
        \be
        \bar{\mathbf{L}}^{\mathfrak{n}+1} = [\bar{\mathbf{L}}^{\mathfrak{n}+1}_{cons}, \bar{\mathbf{L}}^{\mathfrak{n}+1}_{rem}],
        \ee
        where $\bar{\mathbf{L}}^{\mathfrak{n}+1}_{cons} \in \mathbb{R}^{n\times 1}$, $\bar{\mathbf{L}}^{\mathfrak{n}+1}_{rem} \in \mathbb{R}^{n\times r'}$.
        \item Apply the decomposition Algorithm \ref{qrw} to $\bar{\mathbf{L}}^{\mathfrak{n}+1}_1$ and obtain
        \be
        \bar{\mathbf{L}}^{\mathfrak{n}+1}_{cons} = E^{\mathfrak{n}+1}_{cons} S^{\mathfrak{n}+1}_{cons}.
        \ee
        \item Apply the decomposition Algorithm \ref{qrw} to $\bar{\mathbf{L}}^{\mathfrak{n}+1}_{rem}$, and obtain
        \be
        \bar{\mathbf{L}}^{\mathfrak{n}+1}_{rem} = \bar E^{\mathfrak{n}+1}_{rem} \bar S^{\mathfrak{n}+1}_{rem}.
        \ee
        \item  Apply the SVD decomposition to $\bar S^{\mathfrak{n}+1}_{rem}$ and truncate $S^{\mathfrak{n}+1}_{rem} \in \mathbb{R}^{(r'-1)\times (r'-1)}$,
       \be
       \bar S^{\mathfrak{n}+1}_{rem} \approx U^* S^{\mathfrak{n}+1}_{rem} (E^*)^T,
       \ee
       and compute 
       \be
       U^{\mathfrak{n}+1}_{rem} = \tilde U^{\mathfrak{n}+1}_{rem} U^*, \quad E^{\mathfrak{n}+1}_{rem} = \bar E^{\mathfrak{n}+1}_{rem} E^*.
       \ee
       \item Set $U^{\mathfrak{n}+1} = [U^\teq, U^{\mathfrak{n}+1}_{rem}]$.
      \item Set $\bar E^{\mathfrak{n}+1} = [E^{\mathfrak{n}+1}_{cons}, E^{\mathfrak{n}+1}_{rem}]$ and apply Algorithm \ref{qrw} and obtain
      \be
      \bar E^{\mathfrak{n}+1}=E^{\mathfrak{n}+1} R^{\mathfrak{n}+1}.
      \ee
      \item Set 
      \begin{equation}
S^{\mathfrak{n}+1} = 
\begin{bmatrix}
S^{\mathfrak{n}+1}_{cons} & 0 \\
0 & S^{\mathfrak{n}+1}_{rem} \\
\end{bmatrix}
(R^{\mathfrak{n}+1})^T.
\end{equation}
   \end{itemize}
\fi
\end{itemize}
\end{alg}

Both Algorithm \ref{lralgctp2E} and Algorithm \ref{lralgctp21} are conservative, we delay the proof to the next section. However, they may introduce truncation errors in decomposition (\ref{trunerr}).
For isotropic kernel ($M = 0$), conservation of the zeroth moment is enough to guarantee the solution converges to the equilibrium solution. However, for an anisotropic kernel with $M\geq 1$, the conservation of the zeroth moment does not guarantee the solution converges to the correct equilibrium solution. Extra basis functions except $U^\teq$ may be needed to ensure the $\ell$th moment ($\ell \geq 1$) decays to zero.

\subsection{A truncation conservative and error-free algorithm}
In the following, we propose a new algorithm that can avoid truncation errors and converges to the equilibrium solution.
%For equation (\ref{tp2}) with isotropic isoenergetic scattering kernel ($M=0$) and anisotropic one ($M\geq 1$), we will take different strategies to remedy the Algorithm \ref{lralg} such that the solution conserves the total number of the particles. 

We denote by 
\be\label{UeqlIso}
\bal
U^\teq_0 = & U^\teq, \\
U^\teq_\ell = & \frac{1}{\|L_\ell\|}L_\ell, \quad 1 \leq \ell \leq M,
\eal
\ee
where $U^\teq$ is defined in (\ref{USEeq}a). 
Then (\ref{tp2kstep3}) can be rewritten as
\be\label{tp2kstep31}
\bal
\mathbf{K}^{\mathfrak{n}+1}  
%= & \left( U^\mathfrak{n}S^\mathfrak{n} + 2\pi\Delta t \sum_{l=0}^M L_{\ell} \left(\widetilde{\mathbf{K}}^{\mathfrak{n}+1}_\ell \widetilde{A}_\ell^{\Iso,\mathfrak{n}}\right) \right)\left(I_{r}+ 4\pi \Delta t \widetilde{A}_0^{\Iso,\mathfrak{n}} \right)^{-1}
=  U^\mathfrak{n} \bar S^\mathfrak{n} + \sum_{\ell=0}^M U^\teq_{\ell} \bar{\mathbf{K}}^{\mathfrak{n}+1}_\ell,
\eal
\ee
where 
\be
\bar{S}^{\mathfrak{n}} = S^{\mathfrak{n}} \left(I_{r}+ 4\pi \Delta t \widetilde{A}_0^{\Iso,\mathfrak{n}} \right)^{-1} \in \mathbb{R}^{r\times r},
\ee
and
\be
\bar{\mathbf{K}}^{\mathfrak{n}+1}_\ell = 2\pi\Delta t \|L_\ell\|\left(\widetilde{\mathbf{K}}^{\mathfrak{n}+1}_\ell \widetilde{A}_\ell^{\Iso,\mathfrak{n}}\right) \left(I_{r}+ 4\pi \Delta t \widetilde{A}_0^{\Iso,\mathfrak{n}} \right)^{-1} \in \mathbb{R}^{1\times r}.
\ee

%We assume that $U^\mathfrak{n}=[U^\teq, U^\mathfrak{n}_{rem}]$, and $S^\mathfrak{n}=[(S^\mathfrak{n}_1)^T, (S^\mathfrak{n}_{rem})^T]^T$ with $S^\mathfrak{n}_1 \in \mathbb{R}^{r\times 1}$ and $S^\mathfrak{n}_{rem} \in \mathbb{R}^{r\times (r-1)}$. 

We can see from the right-hand side of (\ref{tp2kstep31}) that $M+1$ basis functions $U_\ell^\teq$ are combined with the previous step base $U^\mathfrak{n}$ to generate the new base $U^{\mathfrak{n}+1}$. Similar to Lemma \ref{EMinU}, we have the following result.
\begin{lemma}\label{IsoinU}
Let $U^\mathfrak{n}$ be the base in Algorithm \ref{lralg} for Eq. (\ref{tp2}) and $U^\teq_\ell$ be the unit vector given by (\ref{UeqlIso}). If $\|(U^{\eq}_\ell)^T U^{\mathfrak{n}}\|=1$, then it follows
\be
\|(U^{\eq})^T U^{\mathfrak{n}+1}\|=1,
\ee
and there exists a unitary matrix $V$ such that
\be\label{un1un+}
U^{\mathfrak{n}+1} = U^{\mathfrak{n}} V.
\ee
\end{lemma}

Lemma \ref{IsoinU} indicates that we can prepare $U^0$ such that $\|(U^\teq)^TU^0\|=1$, then we can always choose the base $U^\mathfrak{n}=U^0$, so that we can skip solving the K-step.


If one element has already in the basis, then it won't change other elements, otherwise, the elements including $U^\teq$ will be changed.
We may also design a K-step free and truncation error-free algorithm by adding the elements 
$U^\teq_\ell$ 
into the initial basis $U^0$.

\begin{alg}\label{lralgctp2M}
A K-step free, truncation error free, conservative, and implicit unconventional integrator for equation (\ref{tp2}) with the isotropic scattering kernel ($M\geq 1$):
\begin{itemize}
\item{\textbf{Step 1:}} (Initialization) Given initial basis $U^0$ with rank $r$, set $r'=r$.\\
For $\ell = 0,\cdots, M$, set $\mathbf{K}^0=[U^0, U^\teq_\ell]$. 
\begin{itemize}
    \item If $\text{rank}(U^0) < \text{rank}(\mathbf{K}^0)$, perform a QR factorization $\mathbf{K}^0=U^0R^0$, and set $r'=r'+1$.
\end{itemize}
  Compute the $(r+1)\times r$ matrix $M^0=(U^0)^T(U^0)'$, and set $S^0 = M^0(S^0)'$.
    \item{\textbf{Step 2-4:}} They are similar to Step 2-4 in Algorithm \ref{lralgctp20}, with only a difference in dimension.
\end{itemize}
\end{alg}

\begin{alg}\label{lralgctp20}
A K-step free, truncation error-free and conservative semi-implicit unconventional integrator for Eq. (\ref{tp2}) with the isotropic scattering kernel ($M=0$):
\begin{itemize}
\item{\textbf{Step 1:}} The same initialization as Algorithm \ref{lralgtp1} Step 1.
    \item{\textbf{Step 2:}} Choose $\tilde U^{\mathfrak{n}+1}=U^0$ and 
update $E^\mathfrak{n} \rightarrow \tilde E^{\mathfrak{n}+1}$:
\begin{itemize}
    \item{\textbf{L-step}:} Solve the $n\times r'$ matrix equation (\ref{lstep});\\
    Set $\tilde{\mathbf{L}}^{\mathfrak{n}+1} = [\mathbf{L}^{\mathfrak{n}+1}, E^\mathfrak{n}]$; \\
    Perform decomposition in Algorithm \ref{qrw} such that  $\tilde{\mathbf{L}}^{\mathfrak{n}+1}= \tilde{E}^{\mathfrak{n}+1} \tilde{R}^{\mathfrak{n}+1}$, and compute the $2r' \times r'$ matrix $N^{\mathfrak{n}+1}=(\tilde E^{\mathfrak{n}+1})^T A_\varepsilon E^\mathfrak{n}$.
\end{itemize}
   \item{\textbf{Step 3:}} Update $S^\mathfrak{n}\rightarrow \tilde S^{\mathfrak{n}+1}$:
   \begin{itemize}
       \item{\textbf{S-step}:} Solve the $r'\times 2r'$ matrix equation (\ref{sstep}) with $S^{\mathfrak{n}+1}$ replaced by $\tilde S^{\mathfrak{n}+1}$ and $M^{\mathfrak{n}+1}=(\tilde U^{\mathfrak{n}+1})^TU^{\mathfrak{n}}$.
   \end{itemize}
   \item{\textbf{Step 4:}} Truncate the basis  $\tilde{E}^{\mathfrak{n}+1} \rightarrow {E}^{\mathfrak{n}+1}$.
   \begin{itemize}
       \item  Apply the SVD decomposition to $\tilde S^{\mathfrak{n}+1}$ and truncate $S^{\mathfrak{n}+1} \in \mathbb{R}^{r'\times r'}$,
       $$
       \tilde S^{\mathfrak{n}+1} = U^* S^{\mathfrak{n}+1} (E^*)^T;
       $$
      \item Set $U^{\mathfrak{n}+1} = \tilde{U}^{\mathfrak{n}+1} U^*$, and $E^{\mathfrak{n}+1} = \tilde{E}^{\mathfrak{n}+1} E^*$.
   \end{itemize}
\end{itemize}
\end{alg}

\begin{remark}\label{notrunctionerror}
In Algorithm \ref{lralgctp20}, since $\text{rank}(\tilde S^{\mathfrak{n}+1}) \leq r'$, so Step 4 has no truncation error, namely,
\be\label{notruncation}
U^{\mathfrak{n}+1}S^{\mathfrak{n}+1} (E^{\mathfrak{n}+1})^T = \tilde{U}^{\mathfrak{n}+1} \tilde S^{\mathfrak{n}+1} (\tilde{E}^{\mathfrak{n}+1})^T,
\ee
\end{remark}

For L-step in Algorithm \ref{lralgctp20}, we have
\be\label{tLVEL}
\tilde{\mathbf{L}}^{\mathfrak{n}+1} \tilde V = [E^\mathfrak{n}, \mathbf{L}^{\mathfrak{n}+1}],
\ee
where the unitary matrix $\tilde V=[0, I_{r'}; I_{r'}, 0]$.
The decomposition to $\tilde{\mathbf{L}}^{\mathfrak{n}+1}\tilde V$ gives 
\be\label{ELEE}
[E^\mathfrak{n}, \mathbf{L}^{\mathfrak{n}+1}] = [E^\mathfrak{n}, (E^{\mathfrak{n}+1})']R,
\ee
with $(E^\mathfrak{n})^T A_\varepsilon (E^{\mathfrak{n}+1})'=0$. (\ref{tLVEL}) and (\ref{ELEE}) give
\be
\tilde{\mathbf{L}}^{\mathfrak{n}+1}  = [E^\mathfrak{n}, (E^{\mathfrak{n}+1})']R\tilde V^T,
\ee
Therefore, the basis $\tilde{E}^{\mathfrak{n}+1}$ in L-step satisfies
\be
\tilde{E}^{\mathfrak{n}+1} = [E^\mathfrak{n}, (E^{\mathfrak{n}+1})'] V,
\ee
where $V=[V_1^T, V_2^T]^T\in \mathbb{R}^{2r'\times 2r'}$ is a unitary matrix. Thus, we have
\be
(E^\mathfrak{n})^T A_\varepsilon \tilde{E}^{\mathfrak{n}+1} = [I_{r'}, 0][V_1^T, V_2^T]^T = V_1 \in \mathbb{R}^{r'\times 2r'}.
\ee
Namely, the condition of Lemma \ref{Ebasis} is satisfied.


%For the isotropic case ($M=0$), we have the following result similar to Lemma \ref{EMinU}.



By Lemma \ref{Ubasis} and Lemma \ref{Ebasis}, we have the following result.
\begin{theorem}\label{ptccons0}
Let $U^{\mathfrak{n}}$ and $E^{\mathfrak{n}}$ be the basis in Algorithm \ref{lralgctp20} for equation (\ref{tp2}), if they satisfy the conditions in Lemma \ref{Ubasis} and Lemma \ref{Ebasis}, then the dynamical low-rank DG solution $\hat f_h^{\mathfrak{n}}$ conserves the zeroth moment
\be\label{zeromom}
\hat m^\mathfrak{n}_{0h} = \hat m^0_{0h},
\ee
therefore, it also conserves the total number of particles, namely,
\be\label{ptcformula}
\int_{\Omega_\varepsilon}\int_{\Omega_\mu} \hat f_h^{\mathfrak{n}} d\mu dV_{\varepsilon} = \int_{\Omega_\varepsilon}\int_{\Omega_\mu} \hat f_h^0 d\mu dV_{\varepsilon}, \quad \forall \mathfrak{n}.
\ee
\end{theorem}
\begin{proof}
Recall that for $\hat f_h^\mathfrak{n} = X^T(\mu) \hat F^\mathfrak{n} Y(\varepsilon)$, the zeroth moment has the form
\be\label{zeroth}
\hat m_{0h}^\mathfrak{n} = \frac{1}{2} \int_{\Omega_\mu} \hat f_h^{\mathfrak{n}} d\mu = \frac{1}{2} L_0^T \hat{F}^\mathfrak{n}Y(\varepsilon),
\ee
and the total number of the particles is given by
\be\label{fntomat+}
\bal
\int_{\Omega_\varepsilon}\int_{\Omega_\mu} \hat f_h^{\mathfrak{n}} d\mu dV_{\varepsilon} 
%= & \int_{\Omega_\varepsilon}\int_{\Omega_\mu} X^T(\mu) \hat F^\mathfrak{n} Y(\varepsilon) d\mu dV_{\varepsilon} 
=  \int_{\Omega_\varepsilon}\left(\int_{\Omega_\mu} X^T(\mu) d\mu \right) \hat F^{\mathfrak{n}} Y(\varepsilon) dV_{\varepsilon}
=  \int_{\Omega_\varepsilon}L_{0}^T \hat F^{\mathfrak{n}} Y(\varepsilon) dV_{\varepsilon} = 2\int_{\Omega_\varepsilon} \hat m_{0h}^\mathfrak{n} dV_\varepsilon.
\eal
\ee
Note that
\be\label{lrptcf}
\bal
L_0^T \hat F^{\mathfrak{n}+1} = &  L_0^T U^{\mathfrak{n}+1}S^{\mathfrak{n}+1} (E^{\mathfrak{n}+1})^T \\
= & L_0^T \tilde U^{\mathfrak{n}+1}\tilde S^{\mathfrak{n}+1} (\tilde E^{\mathfrak{n}+1})^T \quad\quad \text{(by Remark \ref{notrunctionerror})} \\
= & L_0^T \tilde U^{\mathfrak{n}+1}{\tilde{\mathbf{S}}}^{\mathfrak{n}} (\tilde E^{\mathfrak{n}+1})^T \quad\quad \text{(by Lemma \ref{Ubasis})} \\
= & \|L_0\| (U^\teq)^T \tilde U^{\mathfrak{n}+1}   (\tilde U^{\mathfrak{n}+1})^T U^{\mathfrak{n}} {S}^\mathfrak{n} (E^{\mathfrak{n}})^T A_{\varepsilon}\tilde E^{\mathfrak{n}+1}(\tilde E^{\mathfrak{n}+1})^T  \\
= &  \|L_0\| (U^\teq)^T U^{\mathfrak{n}} {S}^\mathfrak{n} (E^{\mathfrak{n}})^T \quad\quad \text{(by Lemma \ref{uequn} and Lemma \ref{Ebasis})} \\
= & L_0^T U^{\mathfrak{n}} {S}^\mathfrak{n} (E^{\mathfrak{n}})^T = L_0^T \hat F^{\mathfrak{n}},
\eal
\ee
where ${\tilde{\mathbf{S}}}^{\mathfrak{n}} = (\tilde U^{\mathfrak{n}+1})^T U^{\mathfrak{n}} {S}^\mathfrak{n} (E^{\mathfrak{n}})^T A_{\varepsilon}\tilde E^{\mathfrak{n}+1}$.
Applying (\ref{lrptcf}) for all $\mathfrak{n}$, we have
$$
L_{0}^T \hat  F^\mathfrak{n} = L_{0}^T \hat F^{\mathfrak{n}-1} = \cdots = L_{0}^T \hat F^0.
$$
Thus, (\ref{zeroth}) gives
\be
\hat m_{0h}^\mathfrak{n} = \frac{1}{2} L_0^T \hat{F}^\mathfrak{n}Y(\varepsilon) = \frac{1}{2} L_0^T \hat{F}^0Y(\varepsilon) = \hat m_{0h}^0,
\ee
which together with (\ref{fntomat+}) gives 
\be\label{fntomat1+}
\bal
\int_{\Omega_\varepsilon}\int_{\Omega_\mu} \hat f_h^\mathfrak{n} d\mu dV_{\varepsilon} 
= 2\int_{\Omega_\varepsilon} \hat m_{0h}^\mathfrak{n} dV_\varepsilon
=  2\int_{\Omega_\varepsilon} \hat m_{0h}^0 dV_\varepsilon
=\int_{\Omega_\varepsilon}\int_{\Omega_\mu} \hat f_h^0 d\mu dV_{\varepsilon}.
\eal
\ee
\end{proof}

Similar to Lemma \ref{ptccons0}, we can also prove that the solution of Algorithm \ref{lralgctp2M} conserves the total number of particles. However, when $M$ is too large, its computational complexity may be comparable to or larger than that of Algorithm \ref{lralgctp2E}, so one need to balance between truncation error free and not. 

\begin{lemma}\label{ptccons1}
Let $U^{\mathfrak{n}}$ and $E^{\mathfrak{n}}$ be the basis in Algorithm \ref{lralgctp21} for equation (\ref{tp2}), then the dynamical low-rank DG solution $\hat f_h^{\mathfrak{n}}$ conserves the zeroth moment (\ref{zeromom}) as well as the total number of particles (\ref{ptcformula}).
\end{lemma}
\begin{proof}
Similar to the proof of Lemma \ref{ptccons0}, we only need to show 
\be\label{LFF}
L_0^T \hat F^{\mathfrak{n}+1} = L_0^T \hat F^{\mathfrak{n}}.
\ee
Based on Step 4 in Algorithm \ref{lralgctp21}, we have
\be\label{LFn1L}
\bal
L_0^T \hat F^{\mathfrak{n}+1} = &  L_0^T U^{\mathfrak{n}+1}S^{\mathfrak{n}+1} (E^{\mathfrak{n}+1})^T 
=  \|L_0\| \mathbf{e}_1^T S^{\mathfrak{n}+1} (E^{\mathfrak{n}+1})^T = \|L_0\| S^{\mathfrak{n}+1}_{cons} (E^{\mathfrak{n}+1}_{cons})^T \\
= & \|L_0\| (\bar{\mathbf{L}}^{\mathfrak{n}+1}_{cons})^T,
\eal
\ee
where we have used (\ref{EbarE}), (\ref{Sn1decom}), and (\ref{Lconsdecom}).

Similar to (\ref{lrptcf}), we can also prove
\be\label{LFnL}
L_0^T \hat F^{\mathfrak{n}}=L_0^T \tilde U^{\mathfrak{n}+1}\tilde S^{\mathfrak{n}+1} (\tilde E^{\mathfrak{n}+1})^T =\|L_0\| \mathbf{e}_1^T\tilde S^{\mathfrak{n}+1} (\tilde E^{\mathfrak{n}+1})^T = \|L_0\| \mathbf{e}_1^T (\bar{\mathbf{L}}^{\mathfrak{n}+1})^T = \|L_0\|(\bar{\mathbf{L}}^{\mathfrak{n}+1}_{cons})^T.
\ee
where we have used (\ref{LLL}).

(\ref{LFn1L}) and (\ref{LFnL}) gives (\ref{LFF}), which leads to the conclusion.
\end{proof}

\subsection{Equilibrium of Algorithm \ref{lralgctp2M}}

%[[[]Prove conservation properties.  Then prove convergence to equilibrium for our method.]]]

Recall that we denote the coefficient vector of the Legendre polynomial $P_\ell$ with respect to the orthonormal basis $X(\mu)$ by
\be\label{Lmuvec}
L_{\ell} = (P_\ell(\mu), X(\mu))_{\Omega_\mu}= (\Pi P_\ell(\mu), X(\mu))_{\Omega_\mu} \in \mathbb{R}^{m\times 1},
\ee
which follows by Lemma \ref{basisproperty} and (\ref{PiPlerr}) satisfying
\be\label{Lmulprop}
\bal
L_{\ell}^T L_{\ell'} = & (\Pi P_\ell, P_{\ell'})_{L^2(\Omega_\mu)} =  \frac{2}{2\ell+1}\delta_{\ell \ell'}, \quad \ell, \ell' \in [0,k],\\
|L_{\ell}^T L_{\ell'} |= & \left|(\Pi P_\ell, P_{\ell'})_{L^2(\Omega_\mu)}\right|  \leq  \frac{2}{2\ell+1}\delta_{\ell \ell'} + \tau, \quad \ell, \ell' \in [k+1,M],
\eal
\ee
where $\delta_{\ell\ell'}$ is the Kronecker delta function and $\tau$ is the projection error bound in (\ref{Plprojerr}).

By (\ref{Lmuvec}), the $\ell$th moment of $f_h$ can be expanded with respect to the basis $Y(\varepsilon)$ as
\be\label{fhexpress}
m_{\ell h}(\varepsilon) =  \frac{1}{2}\int_{\Omega_\mu}P_\ell(\mu) f_h(\mu,\varepsilon)d\mu = \frac{1}{2} \left(\int_{\Omega_\mu}P_\ell(\mu) X^T(\mu) d\mu \right) F Y(\varepsilon) = \frac{1}{2} L_\ell^T F Y(\varepsilon),
\ee
where the vector $\frac{1}{2} L_\ell^T F$ is the coefficient vector of $m_{\ell h}$ with respect to the basis $Y(\varepsilon)$.

By Proposition \ref{fullDG2lem}, it follows that the 
the full rank DG solution $f_h^\mathfrak{n}$ converges to the zeroth moment of the projection $f_h^0 \in V_h$ of the initial solution,
\be\label{eqiso}
f_h^\teq = m_{0h}^0.
\ee
From (\ref{isopartcons}), if we further truncate the initial data as $\hat f_h^0 \in V_h$, then 
the equilibrium solution in (\ref{eqiso}) will become
\be\label{eqisom}
f_h^\teq = \hat m_{0h}^0 = \frac{1}{2}\int_{\Omega_\mu} \hat f_h^0 d\mu.
\ee
We denote by $\hat f_h^\teq = X(\mu)^T\hat F^\teq Y(\varepsilon)$, then we have by Proposition \ref{prop2.2},
\be
F^\teq = \frac{1}{2} L_0L_0^T \hat F^0.
\ee

By Theorem \ref{ptccons0}, we have the dynamical low rank DG solution of Algorithm \ref{lralgctp2M} conserves the total number of particles. Next, we will show that the solution also converges to the expected equilibrium solution (\ref{eqisom}) as $\Delta t \rightarrow \infty$.
Recall that $f_h^\teq = X(\mu)^T F^\teq Y(\varepsilon)$ with 
\be\label{Feqiso}
F^\teq = \frac{1}{2} L_0L_0^T \hat F^0 = U^{\teq} S^\teq (E^\teq)^T,
\ee
where $U^\teq$ is given by (\ref{USEeq}a) or (\ref{Ueql0Iso}), and
\begin{subequations}\label{USEeqiso}
\begin{align}
E^\teq = & \frac{1}{ \sqrt{L_0^T \hat F^0 A_\varepsilon (\hat F^0)^T L_0  } } (\hat F^0)^T L_0  \in \mathbb{R}^{n\times 1},\\
S^\teq = & \left[\frac{1}{2}\|L_0\| \sqrt{ L_0^T \hat F^0 A_\varepsilon (\hat F^0)^T L_0  } \right] \in \mathbb{R}^{1\times 1},
\end{align}
\end{subequations}
Here, the basis $U^\teq$ and $E^\teq$ also satisfy (\ref{leqprop}) and (\ref{Eeqorth}).
Let $f_{S^\mathfrak{n}}^\teq$ be the piecewise weighted $L^2$ projection of the equilibrium approximation $f_h^\teq$ in the subspace $V_{S^{\mathfrak{n}}}$, then it can be expressed as (\ref{feqsnproj1}), namely,
\be\label{feqsnprojiso1}
f_{S^{\mathfrak{n}}}^{\text{eq}} = X(\mu)U^{\mathfrak{n}}(U^{\mathfrak{n}})^TF^\teq A_\varepsilon E^{\mathfrak{n}}(E^{\mathfrak{n}})^T Y(\varepsilon) \in V_{S^{\mathfrak{n}}}.
\ee

\begin{lemma}
The matrix $S^\teq$ is uniformly bounded in the following sense,
\be
\|S^\teq\| \leq \sqrt{2}\|f_0\|_{L^2(\Omega)}.
\ee
\end{lemma}
\begin{proof}
Similar to the proof of Lemma \ref{seqbddlem}, we have
\be
\|S^\teq\|^2 = \|\varepsilon \hat f_h^\teq\|^2_{L^2(\Omega)} = \|\varepsilon \hat m_{0h}^0 \|^2_{L^2(\Omega)} = 2 \|\hat f_h^0\|^2_{L^2(\Omega)} \leq 2 \|f_0\|^2_{L^2(\Omega)}.
\ee
\end{proof}

\begin{lemma}\label{RquolemIso}
Let $m'$ be an integer satisfying $1 \leq m' \leq m$ and $Z \in \mathbb{R}^{m'\times n}$ be any nonzero matrices, then it follows
\begin{subequations}\label{RalquoIso}
\begin{align}
R'_{\min} \leq & \frac{(Z\left( A^{\Iso}_0 - \frac{1}{2l+1} A^{\Iso}_\ell \right),Z)_\mathcal{F}}{(ZA_\varepsilon,Z)_\mathcal{F}} \leq R'_{\max},\\
\frac{1}{R'_{\max}}  \leq & \frac{(Z\left( A^{\Iso}_0 - \frac{1}{2l+1} A^{\Iso}_\ell \right)^{-1},Z)_\mathcal{F}}{(ZA_\varepsilon^{-1},Z)_\mathcal{F}} \leq \frac{1}{R'_{\min}},
\end{align}
\end{subequations}
\end{lemma}
Let $(\lambda , q)$ be an eigenpair of the matrix $C_\varepsilon \left( A^{\Iso}_0 - \frac{1}{2l+1} A^{\Iso}_\ell \right)^{-1} C^{T}_\varepsilon$, where $q \in \mathbb{R}^{n \times 1}$. 
From the proof of Lemma \ref{Rquolem}, we have $\frac{1}{R'_{\max}} \leq \lambda \leq \frac{1}{R'_{\min}}$, and
\be\label{AAeigIso}
C_\varepsilon \left( A^{\Iso}_0 - \frac{1}{2l+1} A^{\Iso}_\ell \right)^{-1} C^{T}_\varepsilon q = \lambda q.
\ee
Let $\bar{q} = (C_\varepsilon)^{-1} q$, then (\ref{AAeig}) is equilvalent to 
\be\label{AAeig1Iso}
\left( A^{\Iso}_0 - \frac{1}{2l+1} A^{\Iso}_\ell \right)^{-1} A_\varepsilon \bar q = \lambda \bar q,
\ee
which implies that $\lambda$ is also an eigenvalue of the matrix $\left( A^{\Iso}_0 - \frac{1}{2l+1} A^{\Iso}_\ell \right)^{-1} A_\varepsilon$.
Similarly, the eigenvalue $\lambda$ of $D_\varepsilon=C^{-T}_\varepsilon \left( A^{\Iso}_0 - \frac{1}{2} \|\Pi P_\ell\|^2_{(L^2(S^1))} A^{\Iso}_\ell \right) C^{-1}_\varepsilon$ satisfies
\be\label{eigAiAo}
R'_{\min} \leq \lambda \leq R'_{\max}.
\ee
Similarly, we have the eigenvalue of the matrix $\lambda$ of $A^{-1}_\varepsilon \left( A^{\Iso}_0 - \frac{1}{2} \|\Pi P_\ell\|^2_{(L^2(S^1))} A^{\Iso}_\ell \right)$ satisfies (\ref{eigAiAo}).
\begin{lemma}\label{basisiosproj}
Let $U^\mathfrak{n}$ and $E^\mathfrak{n}$ be the basis in Algorithm \ref{lralgctp2M}.
For some given constant $\beta \in (0,1]$, we assume that 
\be\label{EeqEnIso}
\|(E^\teq)^T A_\varepsilon E^\mathfrak{n}\| \geq \beta,
\ee
then for any $\delta > 0$, there exists $t_*=\frac{\sqrt{r}\gamma}{\beta\|S^\teq\|\delta }$ with 
\be\label{gamma}
\gamma=\left( \frac{1}{4\pi \min_{\varepsilon \in \Omega_\varepsilon}  R_0(\varepsilon) } + \alpha \frac{\max_{\ell}\|R_\ell\|_{L^\infty(\Omega_\varepsilon)}}{\min_{\varepsilon \in \Omega_\varepsilon} R_0(\varepsilon) } \right),
\ee
and $\alpha$ given in (\ref{ratioriso}),
such that when $\Delta t \geq t_*$ it follows
\be\label{eaeiso}
1-\|(E^\teq)^T A_\varepsilon E^{\mathfrak{n}+1}\|^2 \leq \delta^2\|\varepsilon(\hat{f}_h^{\mathfrak{n}}- f^\teq_h) \|_{L^2(\Omega)}^2.
\ee
Moreover, if $\hat{f}_h^\mathfrak{n}=f_h^\teq$, then for any $\Delta t>0$, if follows
\be\label{UUEEasumpt1Iso}
\|(E^\teq)^T A_\varepsilon E^{\mathfrak{n}+1}\| =1.
\ee
\end{lemma}

\begin{proof}
The matrix equation of (\ref{fullDG1K}b) for equation (\ref{tp2}) is equivalent to find $\mathbf{L}^{\mathfrak{n}+1} \in \mathbb{R}^{n\times r}$ such that for any $\mathbf{L}_W\in \mathbb{R}^{n\times r}$,
\be\label{halfmatodeKisob}
\bal
& \left(U^\mathfrak{n} \left(  \frac{\mathbf{L}^{\mathfrak{n}+1} - \mathbf{L}^\mathfrak{n}}{\Delta t} \right)^T A_{\varepsilon}, U^\mathfrak{n}\mathbf{L}_W^T \right)_\mathcal{F}
=  \left(2\pi \sum_{\ell=0}^M L_{\ell} L_{\ell}^T F A^{\Iso}_\ell-4\pi U^\mathfrak{n}(\mathbf{L}^{\mathfrak{n}+1})^T A^{\Iso}_0, U^\mathfrak{n}\mathbf{L}_W^T\right)_\mathcal{F}\\
& =  \left(4\pi \left( \frac{1}{2}L_0 L_0^T \hat F^0 - U^\mathfrak{n}(\mathbf{L}^{\mathfrak{n}+1})^T \right) A^{\Iso}_0, U^\mathfrak{n}\mathbf{L}_W^T\right)_\mathcal{F} + \left(2\pi \sum_{\ell=1}^M L_{\ell} L_{\ell}^T U^\mathfrak{n}(\mathbf{L}^{\mathfrak{n}+1})^T A^{\Iso}_\ell, U^\mathfrak{n}\mathbf{L}_W^T\right)_\mathcal{F}.
\eal
\ee
Since $U^\mathfrak{n}$ in Algorithm \ref{lralgctp21} satisfies 
$\|U_\ell^\teq U^\mathfrak{n}\|=1$, then by Lemma \ref{uequn} 
there exists a unitary matrix $V_\ell \in \mathbb{R}^{r' \times r'}$, such that
\be\label{UnVl}
U^\mathfrak{n} V_\ell= [U^\teq_\ell, U^\teq_{\ell, rem}],
\ee
where $U^\teq_\ell \in \mathbb{R}^{m\times 1}$ and $U^\teq_{\ell, rem} \in \mathbb{R}^{m\times (r'-1)}$.

First, by the arbitrariness of $\mathbf{L}_W$, we take
\be
\mathbf{L}_W = V_\ell [\mathbf{L}_{W_1}, 0]^T,
\ee
where $\mathbf{L}_{W_1} \in \mathbb{R}^{n\times 1}$, then we have
\be\label{UnVUeql}
U^\mathfrak{n}\mathbf{L}_W^T = U^\teq_\ell \mathbf{L}_{W_1}^T.
\ee
By (\ref{UnVUeql}), Lemma \ref{FrobProp} and the arbitrariness of $\mathbf{L}_{W_1}$, we have for $1 \leq \ell \leq k$,
\be
\left((U^\teq_\ell)^TU^\mathfrak{n} \left(  \frac{\mathbf{L}^{\mathfrak{n}+1} - \mathbf{L}^\mathfrak{n}}{\Delta t} \right)^T A_{\varepsilon}, \mathbf{L}_{W_1}^T \right)_\mathcal{F} = \left(4\pi (U^\teq_\ell)^T U^\mathfrak{n}(\mathbf{L}^{\mathfrak{n}+1})^T \left( \frac{1}{2l+1} A^{\Iso}_\ell - A^{\Iso}_0 \right), \mathbf{L}_{W_1}^T\right)_\mathcal{F}.
\ee
By the arbitrariness of $\mathbf{L}_{W_1}$, we have
\be\label{tLn1}
\left(I_n+ 4\pi\Delta t A_\varepsilon^{-1}\left( A^{\Iso}_0 - \frac{1}{2l+1} A^{\Iso}_\ell \right) \right) \tilde{\mathbf{L}}^{\mathfrak{n}+1}_\ell   =  \tilde{\mathbf{L}}^{\mathfrak{n}}_\ell,
\ee
where $\tilde{\mathbf{L}}^{\mathfrak{n}+1}_\ell = \mathbf{L}^{\mathfrak{n}+1} (U^{\mathfrak{n}})^T U^\teq_\ell \in \mathbb{R}^{n\times 1}$ and $\tilde{\mathbf{L}}^{\mathfrak{n}}_\ell =\mathbf{L}^{\mathfrak{n}} (U^{\mathfrak{n}})^T U^\teq_\ell = E^{\mathfrak{n}} (S^{\mathfrak{n}})^T (U^{\mathfrak{n}})^T U^\teq_\ell$. From (\ref{tLn1}), we have
\be
\tilde{\mathbf{L}}^{\mathfrak{n}+1}_\ell =  \left(I_n+ 4\pi\Delta t A_\varepsilon^{-1}\left( A^{\Iso}_0 - \frac{1}{2l+1} A^{\Iso}_\ell \right) \right)^{-1} \tilde{\mathbf{L}}^{\mathfrak{n}}_\ell.
\ee
By (\ref{AAeig1Iso}), we have for $1\leq \ell \leq k$,
\be\label{LALTbdd}
\|C_\varepsilon\tilde{\mathbf{L}}^{\mathfrak{n}+1}_\ell\|^2=\left((\tilde{\mathbf{L}}^{\mathfrak{n}+1}_\ell)^T A_\varepsilon, (\tilde{\mathbf{L}}^{\mathfrak{n}+1}_\ell)^T \right) \leq c^2 \left((\tilde{\mathbf{L}}^{\mathfrak{n}}_\ell)^T A_\varepsilon, (\tilde{\mathbf{L}}^{\mathfrak{n}}_\ell)^T \right)=c^2\|C_\varepsilon\tilde{\mathbf{L}}^{\mathfrak{n}}_\ell\|^2. 
\ee
For $k+1 \leq \ell \leq M$, we have
\be
\bal
& \left((U^\teq_\ell)^TU^\mathfrak{n} \left(  \frac{\mathbf{L}^{\mathfrak{n}+1} - \mathbf{L}^\mathfrak{n}}{\Delta t} \right)^T A_{\varepsilon}, \mathbf{L}_{W_1}^T \right)_\mathcal{F} =  \left(4\pi (U^\teq_\ell)^T U^\mathfrak{n}(\mathbf{L}^{\mathfrak{n}+1})^T \left( \frac{1}{2} \|\Pi P_\ell\|^2_{(L^2(S^1))} A^{\Iso}_\ell - A^{\Iso}_0 \right), \mathbf{L}_{W_1}^T\right)_\mathcal{F}\\
& + \left(2\pi \sum_{\ell'=1}^M \|L_{\ell'}\|^2_{S^1}  (U_{\ell}^\teq, U^\teq_{\ell'})_{L^2(S^1)} U_{\ell'}^T U^\mathfrak{n}\mathbf{L}^{\mathfrak{n}+1} A^{\Iso}_{\ell'}, \mathbf{L}_{W_1}^T\right)_\mathcal{F}.
\eal
\ee
By the arbitrariness of $\mathbf{L}_{W_1}$, we obtain a linear system for $k+1 \leq \ell \leq M$,
\be\label{tLn1M}
\bal
& \left(I_n+ 4\pi\Delta t A_\varepsilon^{-1}\left( A^{\Iso}_0 - \frac{1}{2} \|\Pi P_\ell\|^2_{(L^2(S^1))} A^{\Iso}_\ell \right) \right) \tilde{\mathbf{L}}^{\mathfrak{n}+1}_\ell \\
& - 2\pi\Delta t \sum_{\ell'=k+1, \ell' \not = \ell}^M  \|L_{\ell'}\|^2_{S^1}  (U_{\ell}^\teq, U^\teq_{\ell'})_{L^2(S^1)} A_\varepsilon^{-1} A^{\Iso}_{\ell'} \tilde{\mathbf{L}}^{\mathfrak{n}+1}_{\ell'}  =  \tilde{\mathbf{L}}^{\mathfrak{n}}_\ell.
\eal
\ee
For the linear system (\ref{tLn1M}) and (\ref{LALTbdd}), we have
\be\label{LALTbdd+}
\bal
\sum_{\ell = 1}^M\|C_\varepsilon\tilde{\mathbf{L}}^{\mathfrak{n}+1}_\ell\|
%=  \sum_{\ell = 1}^M\left((\tilde{\mathbf{L}}^{\mathfrak{n}+1}_\ell)^T A_\varepsilon, (\tilde{\mathbf{L}}^{\mathfrak{n}+1}_\ell)^T \right)_\mathcal{F} 
\leq c'\sum_{\ell = 1}^M \|C_\varepsilon\tilde{\mathbf{L}}^{\mathfrak{n}}_\ell\|,
%\leq & c^2\sum_{\ell = 1}^M \left(({\mathbf{L}}^{\mathfrak{n}})^T A_\varepsilon, ({\mathbf{L}}^{\mathfrak{n}})^T \right)_\mathcal{F} = c^2\sum_{\ell = 1}^M\|C_\varepsilon{\mathbf{L}}^{\mathfrak{n}}\|^2,
\eal
\ee
where $c'$ is given by (\ref{ratioriso}). \PY{Will come back to simplify (\ref{LALTbdd+})}
Note that
\be
E^{\teq} (S^\teq)^T (U^\teq)^T  U^\mathfrak{n} (U^{\mathfrak{n}})^T U^\teq_\ell = E^{\teq} (S^\teq)^T (U^\teq)^T  U^\teq_\ell = 0,
\ee
so we have
\be\label{lmombdd}
\tilde{\mathbf{L}}^{\mathfrak{n}}_\ell = (\mathbf{L}^\mathfrak{n}-E^{\teq} (S^\teq)^T (U^\teq)^T  U^\mathfrak{n}) (U^{\mathfrak{n}})^T U^\teq_\ell.
\ee
Note that
\be
\bal
\left((\tilde{\mathbf{L}}^{\mathfrak{n}}_\ell)^T A_\varepsilon, (\tilde{\mathbf{L}}^{\mathfrak{n}}_\ell)^T \right) = &\|C_\varepsilon \tilde{\mathbf{L}}^{\mathfrak{n}}_\ell \|^2 = \|C_\varepsilon \left(\mathbf{L}^\mathfrak{n}-E^{\teq} (S^\teq)^T (U^\teq)^T  U^\mathfrak{n} \right) (U^{\mathfrak{n}})^T U^\teq_\ell\|^2\\
\leq & \|C_\varepsilon \left(\mathbf{L}^\mathfrak{n}-E^{\teq} (S^\teq)^T (U^\teq)^T  U^\mathfrak{n} \right) \|^2_\mathcal{F}.
\eal
\ee


(\ref{LALTbdd+}) and (\ref{lmombdd}) give 
\be\label{LALTbdd0}
\bal
\sum_{\ell = 1}^M\|C_\varepsilon\tilde{\mathbf{L}}^{\mathfrak{n}+1}_\ell\| \leq & c' \sum_{\ell = 1}^M\|C_\varepsilon \left(\mathbf{L}^\mathfrak{n}-E^{\teq} (S^\teq)^T (U^\teq)^T  U^\mathfrak{n} \right) \|^2_\mathcal{F},
\eal
\ee
From (\ref{Lbdd}), we have
\be\label{Lbddiso}
\|C_\varepsilon \left( \mathbf{L}^\mathfrak{n} -  E^{\teq} (S^\teq)^T (U^\teq)^T  U^\mathfrak{n}  \right) \|_{\mathcal{F}} \leq \|\varepsilon(\hat{f}_h^{\mathfrak{n}}- f^\teq_h) \|_{L^2(\Omega)}.
\ee

Next, by taking $\mathbf{L}_W= (A_0^\Iso)^{-1}\mathbf{L}'_W$ in (\ref{halfmatodeKisob}) and applying Lemma \ref{FrobProp}, we have
\be\label{halfmatodeKisob2}
\bal
& \left(\left(  \frac{\mathbf{L}^{\mathfrak{n}+1} - \mathbf{L}^\mathfrak{n}}{\Delta t} \right)^T A_{\varepsilon}(A_0^\Iso)^{-1}, (\mathbf{L}'_W)^T \right)_\mathcal{F} =  \left(4\pi \left( \frac{1}{2} (U^\mathfrak{n})^T L_0 L_0^T \hat F^0 - (\mathbf{L}^{\mathfrak{n}+1})^T \right), (\mathbf{L}'_W)^T\right)_\mathcal{F} \\
& + \left(2\pi \sum_{\ell=1}^M (U^\mathfrak{n})^TL_{\ell} L_{\ell}^T U^\mathfrak{n}(\mathbf{L}^{\mathfrak{n}+1})^T A^{\Iso}_\ell(A_0^\Iso)^{-1}, \mathbf{L}_W^T\right)_\mathcal{F}.
\eal
\ee
By the arbitrariness of $\mathbf{L}'_W$, we have
\be\label{Lforiso}
\bal
& \left(I_n + \frac{1}{4\pi\Delta t}(A_0^\Iso)^{-1}A_{\varepsilon} \right)  \mathbf{L}^{\mathfrak{n}+1} 
%=  E^{\teq} (S^\teq)^T (U^\teq)^T  U^\mathfrak{n}  + \frac{1}{4\pi\Delta t}(A_0^\Iso)^{-1}A_{\varepsilon} \mathbf{L}^{\mathfrak{n}} \\
%& + \frac{1}{2} \sum_{\ell=1}^M (A_0^\Iso)^{-1}A^{\Iso}_\ell \|L_\ell\|^2 \tilde{\mathbf{L}}^{\mathfrak{n}+1}_\ell (U_\ell^\teq)^TU^\mathfrak{n}\\
=  \left(I_n + \frac{1}{4\pi\Delta t}(A_0^\Iso)^{-1}A_{\varepsilon} \right)  E^{\teq} (S^\teq)^T (U^\teq)^T  U^\mathfrak{n} \\
& + \frac{1}{4\pi\Delta t}(A_0^\Iso)^{-1}A_{\varepsilon} \left( \mathbf{L}^{\mathfrak{n}} - E^{\teq} (S^\teq)^T (U^\teq)^T  U^\mathfrak{n}  \right) + \frac{1}{2} \sum_{\ell=1}^M (A_0^\Iso)^{-1}A^{\Iso}_\ell \|L_\ell\|^2 \tilde{\mathbf{L}}^{\mathfrak{n}+1}_\ell (U_\ell^\teq)^TU^\mathfrak{n},
\eal
\ee
where we have used (\ref{Feqiso}).
Therefore, (\ref{Lforiso}) gives
\be
\bal
\mathbf{L}^{\mathfrak{n}+1} = & E^{\teq} (S^\teq)^T (U^\teq)^T  U^\mathfrak{n} +\frac{1}{\Delta t} D_0 \left( \mathbf{L}^{\mathfrak{n}} - E^{\teq} (S^\teq)^T (U^\teq)^T  U^\mathfrak{n}  \right) +\frac{1}{2}  \sum_{\ell=1}^M D_\ell \|L_\ell\|^2 \tilde{\mathbf{L}}^{\mathfrak{n}+1}_\ell (U_\ell^\teq)^TU^\mathfrak{n},
\eal
\ee
where the matrices
\be
D_0 = \frac{1}{4\pi} \left(I_n + \frac{1}{4\pi\Delta t}(A_0^\Iso)^{-1}A_{\varepsilon} \right) ^{-1}(A_0^\Iso)^{-1}A_{\varepsilon},
\ee
and
\be
D_{\ell} = \left(I_n + \frac{1}{4\pi\Delta t}(A_0^\Iso)^{-1}A_{\varepsilon} \right)^{-1} (A_0^\Iso)^{-1}A^{\Iso}_\ell, \quad 1\leq \ell \leq M.
\ee
Next, we have
\be
\bal
& \left((U^\mathfrak{n})^TU_\ell^\teq(\tilde{\mathbf{L}}^{\mathfrak{n}+1}_\ell)^TA_\varepsilon, (U^\mathfrak{n})^TU_\ell^\teq(\tilde{\mathbf{L}}^{\mathfrak{n}+1}_\ell)^T \right) = \left((U_\ell^\teq)^TU^\mathfrak{n}(U^\mathfrak{n})^TU_\ell^\teq, (\tilde{\mathbf{L}}^{\mathfrak{n}+1}_\ell)^T A_\varepsilon \tilde{\mathbf{L}}^{\mathfrak{n}+1}_\ell \right) \\
& \leq \|(U_\ell^\teq)^TU^\mathfrak{n}(U^\mathfrak{n})^TU_\ell^\teq\| \|(\tilde{\mathbf{L}}^{\mathfrak{n}+1}_\ell)^T A_\varepsilon \tilde{\mathbf{L}}^{\mathfrak{n}+1}_\ell\| = \|(\tilde{\mathbf{L}}^{\mathfrak{n}+1}_\ell)^T A_\varepsilon \tilde{\mathbf{L}}^{\mathfrak{n}+1}_\ell\|=\|C_\varepsilon\tilde{\mathbf{L}}^{\mathfrak{n}+1}_\ell\|^2.
\eal
\ee
It is easy to verify that the eigenvalue $\lambda_{D_\ell}$ of $D_\ell$ satisfies
\be
\bal
& 0<\lambda_{D_0} \leq \frac{1}{4\pi \min_{\varepsilon \in \Omega_\varepsilon} R_0(\varepsilon) },\\
& 0<\lambda_{D_\ell} \leq \frac{\|R_\ell\|_{L^\infty(\Omega_\varepsilon)}}{\min_{\varepsilon \in \Omega_\varepsilon} R_0(\varepsilon) }.
\eal
\ee
Let 
\be
B_{\mathbf{L}} = D_0 \left( \mathbf{L}^{\mathfrak{n}} - E^{\teq} (S^\teq)^T (U^\teq)^T  U^\mathfrak{n}  \right) +\frac{1}{2} \Delta t \sum_{\ell=1}^M D_\ell \|L_\ell\|^2 \tilde{\mathbf{L}}^{\mathfrak{n}+1}_\ell (U_\ell^\teq)^TU^\mathfrak{n},
\ee
then we have
\be
\|C_\varepsilon B_{\mathbf{L}}\|_\mathcal{F} \leq \gamma \|\varepsilon(\hat{f}_h^{\mathfrak{n}}- f^\teq_h) \|_{L^2(\Omega)},
\ee
where $\gamma$ is given by (\ref{gamma}).

By (\ref{gamma1eq}), we have as $\Delta t \geq \frac{\sqrt{r}\gamma}{\beta\|S^\teq\|\delta }$, it holds the conclusion (\ref{eaeiso}).
The proof of (\ref{UUEEasumpt1Iso}) is similar to that of Lemma \ref{fsnproj}.
\end{proof}

\begin{corollary}\label{fsnprojiso+} 
Under the conditions of Lemma \ref{basisiosproj},
then for any $\delta > 0$, there exists $t_*=\frac{\sqrt{r}\gamma}{\beta\delta }$ such that when $\Delta t \geq t_*$, it follows
\be\label{Eerroriso}
\|\varepsilon(f_h^{\text{eq}}- f_{S^{\mathfrak{n}+1}}^{\text{eq}})\|_{L^2(\Omega)}  \leq  \delta \|\varepsilon(\hat{f}_h^{\mathfrak{n}}- f^\teq_h) \|_{L^2(\Omega)}.
\ee
Moreover, if $\hat{f}_h^{\mathfrak{n}} = f^\teq_h$, then it follows for any $\Delta t>0$,
\be\label{projeqSiso}
f^\teq_{S^{\mathfrak{n}+1}} = f^\teq_h.
\ee
\end{corollary}
\begin{proof}
From (\ref{htosnproj}) and $\|(U^\teq)^TU^\mathfrak{n}\|=1$, we have for any $\mathfrak{n}$,
\be\label{htosnprojiso}
\bal
& \|\varepsilon(f_h^{\text{eq}}- f_{S^{\mathfrak{n}}}^{\text{eq}})\|_{L^2(\Omega)}^2 =  \|S^\teq\|^2 \left( 1 - \|(E^\teq)^T A_\varepsilon E^{\mathfrak{n}}\|^2 \right).
\eal
\ee
By Lemma \ref{basisiosproj} with $\delta = \frac{\delta'}{\|S^\teq\|}$, we have when $\Delta t \geq \frac{\sqrt{r}\gamma}{\beta \delta'}$, it follows

\be\label{basebddiso0}
1-\|(E^\teq)^T A_\varepsilon E^{\mathfrak{n}+1}\|^2 \leq  \frac{\delta'^2}{\|S^\teq\|^2} \|\varepsilon(\hat{f}_h^{\mathfrak{n}}- f^\teq_h) \|_{L^2(\Omega)}^2.
\ee
Therefore, we have by (\ref{htosnprojiso}) and (\ref{basebddiso0}),
\be
\|\varepsilon(f_h^{\text{eq}}- f_{S^{\mathfrak{n}+1}}^{\text{eq}})\|_{L^2(\Omega)}^2 \leq \delta'^2 \|\varepsilon(\hat{f}_h^{\mathfrak{n}}- f^\teq_h) \|_{L^2(\Omega)}^2.
\ee
The equality (\ref{projeqSiso}) follows from (\ref{UUEEasumpt1Iso}) and (\ref{htosnprojiso}).
\end{proof}

\begin{theorem}\label{LstablemSIso}
Under the conditions of Lemma \ref{basisiosproj},
for any $0<\delta \leq \min\left\{1-c, \frac{\sqrt{1-\beta^2}}{\|\varepsilon (\hat f^{0}_h-f_h^{\text{eq}})\|_{L^2(\Omega)}}\right\}$, 
there exists a constant $t_*=\frac{\sqrt{r}\gamma}{\beta\delta }$ such that when $\Delta t \geq t_*$, it follows
\be\label{LstabSIso}
\bal
\|\varepsilon (\hat f_h^{\mathfrak{n}} - f_h^{\text{eq}})\|_{L^2(\Omega)} \leq &(c+\delta)^\mathfrak{n} \|\varepsilon (\hat f^{0}_h-f_h^{\text{eq}})\|_{L^2(\Omega)},
\eal
\ee
where $c$ is given by (\ref{ratioriso}).

Moreover, if $\hat{f}_h^{0} = f^\teq_h$, then it follows for any $\Delta t>0$,
\be\label{projeqSIso+}
\hat{f}_h^{\mathfrak{n}} = f^\teq_h.
\ee
\end{theorem}

\begin{proof}
For $\forall w_h \in V_{S^{\mathfrak{n}+1}}$, the DG scheme (\ref{fullDG1K}c) for Algorithm \ref{lralgctp21} can be reformulated as
\be\label{fullDG1rSiso}
\left(D_t f_S^{\mathfrak{n}}, w_h;\varepsilon^2 \right)_{\Omega} =4\pi \sum_{l=0}^M \left(\varepsilon^2R_\ell(\varepsilon) \Pi P_\ell(\mu)m_{\ell S}^{\mathfrak{n}+1}(\varepsilon), w_h\right)_{\Omega}-\left(4\pi \varepsilon^2R_0(\varepsilon)f_S^{\mathfrak{n}+1}(\varepsilon, \mu), w_h\right)_{\Omega},
\ee
which is equivalent to find $S^{\mathfrak{n}+1} \in \mathbb{R}^{r\times r}$ such that for any $S_W \in \mathbb{R}^{r\times r}$,
\be\label{Sstepiso}
\bal
& \left(U^{\mathfrak{n}+1}\frac{S^{\mathfrak{n}+1}-\mathbf S^\mathfrak{n}}{\Delta t} (E^{\mathfrak{n}+1})^T A_{\varepsilon}, U^{\mathfrak{n}+1}S_W(E^{\mathfrak{n}+1})^T \right)_\mathcal{F}\\
& =  \left(4\pi \left( \frac{1}{2}L_0 L_0^T \hat F^0 - U^{\mathfrak{n}+1}S^{\mathfrak{n}+1}(E^{\mathfrak{n}+1})^T \right) A^{\Iso}_0, U^{\mathfrak{n}+1}S_W(E^{\mathfrak{n}+1})^T\right)_\mathcal{F} \\
& + \left(2\pi \sum_{\ell=1}^M L_{\ell} L_{\ell}^T U^\mathfrak{n}(\mathbf{L}^{\mathfrak{n}+1})^T A^{\Iso}_\ell, U^{\mathfrak{n}+1}S_W(E^{\mathfrak{n}+1})^T\right)_\mathcal{F}.
\eal
\ee
For Algorithm \ref{lralgctp21}, the basis $U^{\mathfrak{n}+1} = U^{\mathfrak{n}} =\cdots= U^0$, so (\ref{UnVl}) also holds for $U^{\mathfrak{n}+1}$. Therefore, for $V_\ell$ given in (\ref{UnVl}) if we take 
\be\label{SWiso}
S_W = V_\ell [S_{W_1}, 0]^T,
\ee
where $S_{W_1} \in \mathbb{R}^{r\times 1}$ is an arbitrary vector, it follows
\be\label{Un1Sw}
U^{\mathfrak{n}+1}S_W = U^{\mathfrak{n}+1}V_\ell V_\ell^TS_W = U_\ell^\teq S_{W_1}^T. 
\ee
For $S_W$ given by (\ref{SWiso}),  (\ref{Sstepiso}) gives
\be\label{Sstepiso0}
\bal
& \left((U_\ell^\teq)^TU^{\mathfrak{n}+1}\frac{S^{\mathfrak{n}+1}-\mathbf S^\mathfrak{n}}{\Delta t},S_{W_1}^T \right) =  \left(4\pi(U_\ell^\teq)^T U^{\mathfrak{n}+1}S^{\mathfrak{n}+1} \left(\frac{1}{2}\|L_\ell\|^2\widetilde{A}^{\Iso, \mathfrak{n}+1}_{\ell} -\widetilde{A}^{\Iso, \mathfrak{n}+1}_0\right), S_{W_1}^T\right) \\
& + \left(2\pi \sum_{\ell'=1, \ell'\not = \ell}^M (U_\ell^\teq)^T L_{\ell'} L_{\ell'}^T U^{\mathfrak{n}+1}S^{\mathfrak{n}+1} \widetilde{A}^{\Iso, \mathfrak{n}+1}_{\ell'}, S_{W_1}^T\right).
\eal
\ee
By the notation in (\ref{Smoment}), namely, $\widetilde{S}_\ell^{\mathfrak{n}+1} = \|L_\ell\| (U_\ell^\teq)^TU^{\mathfrak{n}+1}S^{\mathfrak{n}+1}$, $\widetilde{\mathbf{S}}_\ell^{n}=\|L_\ell\| (U_\ell^\teq)^T U^{\mathfrak{n}+1}{\mathbf{S}}^{\mathfrak{n}}$, we have for $1\leq \ell \leq M$,
\be\label{Steq}
\bal
& \left(\widetilde{S}_\ell^{\mathfrak{n}+1} \left( I_r + 4\pi\Delta t  \left( \widetilde{A}^{\Iso, \mathfrak{n}+1}_0 -  \frac{1}{2}\|L_\ell\|^2\widetilde{A}^{\Iso, \mathfrak{n}+1}_{\ell} \right) \right), (S'_{W_1})^T\right) \\
& - \left(2\pi \Delta t\sum_{\ell'=1, \ell'\not = \ell}^M L_\ell^T L_{\ell'} \widetilde{S}_{\ell'}^{\mathfrak{n}+1} \widetilde{A}^{\Iso, \mathfrak{n}+1}_{\ell'}, (S'_{W_1})^T\right) = \left(\widetilde{\mathbf{S}}_\ell^{n}, (S'_{W_1})^T\right),
\eal
\ee
where $S'_{W_1} = \frac{1}{\|L_\ell\|}S_{W_1}$. By taking $S'_{W_1} = \widetilde{S}_\ell^{\mathfrak{n}+1}$ in (\ref{Steq}), we obtain
\be\label{salgmat}
\bal
& \sum_{\ell=1}^M \|C_\varepsilon E^{\mathfrak{n}+1} (\widetilde{S}_\ell^{\mathfrak{n}+1})^T\| \leq c' \sum_{\ell=1}^M \|C_\varepsilon E^{\mathfrak{n}+1} (\widetilde{\mathbf{S}}_\ell^{n})^T\| \\
& = c' \sum_{\ell=1}^M \left\|C_\varepsilon E^{\mathfrak{n}+1} \left(({\mathbf{S}}_\ell^{n})^T - (E^{\mathfrak{n}+1})^T A_\varepsilon (F^\teq)^T U^{\mathfrak{n}+1}  \right) (U^{\mathfrak{n}+1})^T L_\ell \right\|,
\eal
\ee
where we have used
\be
(L_\ell)^T U^{\mathfrak{n}+1} (U^{\mathfrak{n}+1})^T F^\teq = (L_\ell)^T F^\teq =0.
\ee
It is easy to verify that
\be
\bal
& \|C_\varepsilon E^{\mathfrak{n}+1} (\widetilde{S}_\ell^{\mathfrak{n}+1})^T\|=2\|\varepsilon \hat m_{\ell h}^{\mathfrak{n}+1}\|, \\
& \left\|C_\varepsilon E^{\mathfrak{n}+1} \left(({\mathbf{S}}_\ell^{n})^T - (E^{\mathfrak{n}+1})^T A_\varepsilon (F^\teq)^T U^{\mathfrak{n}+1}  \right) (U^{\mathfrak{n}+1})^T L_\ell \right\| \\
& \leq \|L_\ell\| \left\|C_\varepsilon E^{\mathfrak{n}+1} \left(({\mathbf{S}}_\ell^{n})^T - (E^{\mathfrak{n}+1})^T A_\varepsilon (F^\teq)^T U^{\mathfrak{n}+1}  \right) (U^{\mathfrak{n}+1})^T \right\|_\mathcal{F}\\
& = \|\Pi P_\ell\|_{L^2(\Omega_\mu)} \|\varepsilon ( \hat f_\mathbf{S}^{\mathfrak{n}} - f^\teq_{S^{\mathfrak{n}+1}}) \|_{L^2(\Omega)}
\eal
\ee
Thus, (\ref{salgmat}) is equivalent to 
\be
\sum_{\ell=1}^M \|\varepsilon \hat m_{\ell h}^{\mathfrak{n}+1} \|_{L^2(\Omega_\varepsilon)} \leq \frac{1}{2} c' \|\varepsilon ( \hat f_\mathbf{S}^{\mathfrak{n}} - f^\teq_{S^{\mathfrak{n}+1}}) \|_{L^2(\Omega)} \sum_{\ell=1}^M \|\Pi P_\ell\|_{L^2(\Omega_\mu)} .
\ee
By Theorem \ref{ptccons0}, we can rewrite (\ref{fullDG1rSiso}) as
\be\label{frdgrelr}
\bal
\left((1+4\pi\Delta t R_0)f_S^{\mathfrak{n}+1}, w_h;\varepsilon^2 \right)_{\Omega} = &  \left( f_{\mathbf{S}}^{\mathfrak{n}}+4\pi\Delta t R_0 \hat m_{0h}^0, w_h; \varepsilon^2\right)_{\Omega} \\
& + 4\pi \Delta t \sum_{l=1}^M \left(R_\ell(\varepsilon) \Pi P_\ell(\mu)m_{\ell S}^{\mathfrak{n}+1}(\varepsilon), w_h;\varepsilon^2\right)_{\Omega}.
\eal
\ee
Subtract $ \left((1+4\pi\Delta t R_0) f^\teq_{S^{\mathfrak{n}+1}}, w_h;\varepsilon^2 \right)_{\Omega} $ from (\ref{frdgrelr}) and set $w_h =f_S^{\mathfrak{n}+1} - f^\teq_{S^{\mathfrak{n}+1}} \in V_{S^{\mathfrak{n}+1}}$, we obtain
\be\label{ffeqbddlr}
\bal
\|\varepsilon ( f_S^{\mathfrak{n}+1} - f^\teq_{S^{\mathfrak{n}+1}} )\|_{L^2(\Omega)} \leq  &  c' \|\varepsilon ( f_\mathbf{S}^{\mathfrak{n}} - f^\teq_{S^{\mathfrak{n}+1}} )\|_{L^2(\Omega)} + 4\pi c'\Delta t \|R_0\|_{L^\infty(\Omega_\varepsilon)}\|\varepsilon(\hat f^\teq_h - f^\teq_{S^{\mathfrak{n}+1}} )\|_{L^2(\Omega)} \\
& +4\sqrt{2}\pi c' \Delta t \max_{\ell} \|R_\ell\|_{L^\infty(\Omega_\varepsilon)} \sum_{\ell=1}^M \|\varepsilon m_{\ell h}^{\mathfrak{n}+1} \|_{L^2(\Omega_\varepsilon)}\\
\leq & c \|\varepsilon ( f_\mathbf{S}^{\mathfrak{n}} - f^\teq_{S^{\mathfrak{n}+1}} )\|_{L^2(\Omega)} + 4\pi c'\Delta t \|R_0\|_{L^\infty(\Omega_\varepsilon)}\|\varepsilon(\hat f^\teq_h - f^\teq_{S^{\mathfrak{n}+1}} )\|_{L^2(\Omega)},
\eal
\ee
where $c$ is given by (\ref{ratioriso}).
By (\ref{fsfeqtri}), (\ref{ctmapping}) and (\ref{ffeqbddlr}), we have
\be\label{LstabSiso+}
\bal
\|\varepsilon (\hat f_h^{\mathfrak{n}+1} - f_h^{\text{eq}})\|_{L^2(\Omega)} \leq & c \|\varepsilon (\hat f_h^{\mathfrak{n}} - f_h^{\text{eq}})\|_{L^2(\Omega)}  + (1+4\pi c'\Delta t \|R_0\|_{L^\infty(\Omega_\varepsilon)}) \|\varepsilon(f_h^{\text{eq}}- f_{S^{\mathfrak{n}+1}}^{\text{eq}})\|_{L^2(\Omega)},
\eal
\ee
By Corollary \ref{fsnprojiso+}, we have that as $\Delta t \geq \frac{\sqrt{r}\gamma(1+4\pi c'\Delta t \|R_0\|_{L^\infty(\Omega_\varepsilon)}) }{\beta\delta }$, we have
\be\label{LstabSiso++}
\bal
\|\varepsilon (\hat f_h^{\mathfrak{n}+1} - f_h^{\text{eq}})\|_{L^2(\Omega)} \leq & (c+\delta) \|\varepsilon (\hat f_h^{\mathfrak{n}} - f_h^{\text{eq}})\|_{L^2(\Omega)}.
\eal
\ee
\PY{will revise here in revision.}
\end{proof}





==> archive/Nonlinear.tex <==
\section{Nonlinear problem (NES)}

At this point, organization of the section is not fixed.

\subsection{Iterative Algorithm}

\subsection{Conservative Fix}

\subsection{Anything else?}
